Presenting a Dataset for Collaborator Recommending Systems in Academic Social Network: a Case Study on ReseachGate

Collaborator finding systems are a special type of expert finding models. There is a long-lasting challenge for research in the collaborator recommending research area, which is the lack of the structured dataset to be used by the researchers. We introduce two datasets to fill this gap. The first dataset is prepared for designing a consistent, collaborator finding system. The next one, called a co-author finding model, models an academic social network as a table that contains different relations between the pair of users. Both of them provide an opportunity for introducing potential collaborators to each other. These two models have been extracted from ResearchGate (RG) data set and are available publicly. RG dataset has been collected from Jan. 2019 to April 2019 and includes raw data of 3980 RG users. The dataset consists of almost complete information about users. In the preprocessing phase, the well-known Elmo was used for analyzing textual data. We call this as ResearchGate dataset for Recommending Systems (RGRS). For assessing the validity of data, we analyze each layer of data separately, and the results are reported. After preparing data and evaluating the collaborator finding models, we have done some assessments on RGRS. Some of these assessments are co-author, following-follower, and question answering relations. The outcomes indicate that it is the best relation in propagating knowledge in the network. To the best of our knowledge, there is no processed and analyzed dataset of this size.

==> base/ltfilehook-code.tex <==
% This will typeset documentation + code
%

\AtBeginDocument{\AlsoImplementation}
\input{ltfilehook.dtx}


==> base/ltfilehook-doc.tex <==
% This will typeset only documentation but not the code
%

\AtBeginDocument{\OnlyDescription
%                 \let\tableofcontents\relax
                 }
\input{ltfilehook.dtx}


==> base/lthooks-code.tex <==
% This will typeset documentation + code
%

\AtBeginDocument{\AlsoImplementation}
\input{lthooks.dtx}


==> base/lthooks-doc.tex <==
% This will typeset only documentation but not the code
%

\AtBeginDocument{\OnlyDescription
%                 \let\tableofcontents\relax
                 }
\input{lthooks.dtx}


==> base/ltshipout-code.tex <==
% This will typeset documentation + code
%

\AtBeginDocument{\AlsoImplementation}
\input{ltshipout.dtx}


==> base/ltshipout-doc.tex <==
% This will typeset only documentation but not the code
%

\AtBeginDocument{\OnlyDescription
%                 \let\tableofcontents\relax
                 }
\input{ltshipout.dtx}


==> base/ltxcheck.tex <==
% \iffalse meta-comment
%
% Copyright (C) 1993-2020
% The LaTeX3 Project and any individual authors listed elsewhere
% in this file.
%
% This file is part of the LaTeX base system.
% -------------------------------------------
%
% It may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3c
% of this license or (at your option) any later version.
% The latest version of this license is in
%    https://www.latex-project.org/lppl.txt
% and version 1.3c or later is part of all distributions of LaTeX
% version 2008 or later.
%
% This file has the LPPL maintenance status "maintained".
%
% The list of all files belonging to the LaTeX base distribution is
% given in the file `manifest.txt'. See also `legal.txt' for additional
% information.
%
% The list of derived (unpacked) files belonging to the distribution
% and covered by LPPL is defined by the unpacking scripts (with
% extension .ins) which are part of the distribution.
%
% \fi
%
% \iffalse
%% File `ltxcheck.tex'.
%% Copyright (C) 1994-1997 LaTeX3 project, David Carlisle
%%
% LaTeX Test File.
% ================
%
% Processing this file with a newly installed LaTeX
% will test various aspects of the installation.
%
% To typeset the comments in this file, create a small
% file ltxcheck.drv that looks like the following (without the %)
%
%    \documentclass{ltxdoc}
%    \begin{document}
%    \DocInput{ltxcheck.tex}
%    \end{document}
%
% and process `latex ltxcheck.drv'.
%
\NeedsTeXFormat{LaTeX2e}[1997/06/01]
% \fi
%
% \StopEventually{}
% \CheckSum{643}
%
% \changes{v1.0c}{1994/03/15}
%         {Add \cmd{\NeedsTeXFormat}}
% \changes{v1.0t}{1996/09/25}
%         {Move ltxcheck to separate file}
% \changes{v1.0v}{1996/11/20}
%         {lowercase filenames /1044}
% \changes{v1.1d}{2004/02/11}
%         {Remove pict2e.sty}
%
\ProvidesFile{ltxcheck.tex}[2015/03/30 v1.1d LaTeX check file (DPC)]
%
% \GetFileInfo{ltxcheck.tex}
% \title{\textsf{ltxcheck}: The \LaTeX\ test program\thanks
%   {version~\fileversion, dated \filedate}}
% \author{David Carlisle}
% \date{\filedate}
% \MaintainedByLaTeXTeam{latex}
% \maketitle
%
% This file, |ltxcheck.tex| should be run after \LaTeX\ has been
% installed. It Checks some system dependent parts of \LaTeX\ are set up
% correctly for your system, and checks that the main input files and
% fonts that \LaTeX\ uses are present and can be found by \LaTeX.
%
%    \begin{macrocode}
\makeatletter
%    \end{macrocode}
%
%    \begin{macrocode}
\typeout{^^J%
LaTeX2e installation check file^^J%
===============================}
%    \end{macrocode}
%
%    \begin{macrocode}
\typeout{^^J%
 Before running this file through LaTeX2e you should have installed^^J%
 the Standard LaTeX files in their final `system' directories.^^J%
 This file should *not* be run in a directory that contains article.cls}
%    \end{macrocode}
%
% |\pause| just slows things down so that not too much appears on the
% screen at once, or scrolls off the top.
%    \begin{macrocode}
\def\pause{%
  \typeout{}%
  \message{** Hit return to continue: }%
  \read -1  to \xxx
  \typeout{}}
%    \end{macrocode}
%
%    \begin{macrocode}
\typeout{^^J%
  After certain tests, LaTeX will pause so that you can read the^^J%
  output without it scrolling off the screen.^^J%
  When you are ready just hit <return> and LaTeX will continue.^^J%
  When LaTeX pauses, you will see a prompt like the one below.^^J^^J%
  If a test fails, a message will be displayed followed by^^J%
  an error message starting `! BAD'.^^J%
  LaTeX will quit if you try to scroll past some error messages.}
\pause
%    \end{macrocode}
%
% Check that the system has defined |\@currdir| correctly
% by writing an |.aux| file and then trying to find it again.
%    \begin{macrocode}
\typeout{^^J%
  Checking the current directory syntax^^J%
  =====================================}
%    \end{macrocode}
%
%    \begin{macrocode}
\newif\iftest\testfalse
%    \end{macrocode}
%
%    \begin{macrocode}
\ifx\@currdir\@undefined
  \typeout{^^J%
  \noexpand\@currdir is undefined !!^^J%
  Something is seriously wrong with the LaTeX2e initialisation.^^J%
  Either you have corrupted files or this is a LaTeX bug.}
  \errmessage{BAD LaTeX2e system!!}
  \expandafter\@@end
\fi
%    \end{macrocode}
%
%    \begin{macrocode}
\ifx\@currdir\@empty
  \typeout{^^J%
  \noexpand\@currdir is defined to be empty.^^J%
  This means that LaTeX can not distinguish between a file^^J%
  aaaaa.tex^^J%
  that exists in the current directory, and  a file aaaaa.tex^^J%
  in another directory.^^J%
  It may be that this Operating System has no concept of `directory'^^J%
  in which case the setting is correct. If however it is possible to^^J%
  uniquely refer to a file then a suitable definition of
    \noexpand\@currdir^^J%
  should be added to texsys.cfg, and the format remade.}
  \pause
%    \end{macrocode}
%
%    \begin{macrocode}
\else
  \typeout{^^J%
\noexpand\@currdir is defined as
    \expandafter\strip@prefix\meaning\@currdir^^J%
  (Testing...)}
%    \end{macrocode}
%
%    \begin{macrocode}
\begingroup
\endlinechar=-1
\count@\time
\divide\count@ 60
\count2=-\count@
\multiply\count2 60
\advance\count2 \time
\edef\today{%
  \the\year/\two@digits{\the\month}/\two@digits{\the\day}:%
    \two@digits{\the\count@}:\two@digits{\the\count2}}
%    \end{macrocode}
%
%    \begin{macrocode}
  \immediate\openout15=ltxcheck.aux
  \immediate\write15{\today^^J}
  \immediate\closeout15 %
%    \end{macrocode}
%
%    \begin{macrocode}
  \openin\@inputcheck\@currdir ltxcheck.aux %
  \ifeof\@inputcheck
    \typeout{\@currdir ltxcheck.aux  not found}%
  \else
    \read\@inputcheck to \reserved@a
    \ifx\reserved@a\today
      \typeout{\@currdir ltxcheck.aux found}
      \testtrue
    \else
      \typeout{BAD: old file \reserved@a(should be \today)}%
      \testfalse
    \fi
  \fi
  \closein\@inputcheck
%    \end{macrocode}
%
%    \begin{macrocode}
  \iftest
    \endgroup
    \typeout{\noexpand \@currdir OK!}
  \else
  \endgroup
%    \end{macrocode}
%
%    \begin{macrocode}
  \typeout{^^J%
    The LaTeX2e installation has defined \noexpand\@currdir^^J%
    to be \expandafter\strip@prefix\meaning\@currdir.^^J%
    This appears to be incorrect.^^J%
    You should add a correct definition to texsys.cfg^^J%
    and rebuild the format.}
  \errmessage{BAD LaTeX2e system!!}
  \expandafter\expandafter\expandafter\@@end
  \fi
  \pause
%    \end{macrocode}
%
%    \begin{macrocode}
\fi
%    \end{macrocode}
%
% \changes{v1.0k}{1995/09/27}
%         {Check filename parser}
% Check the filename parser can at least cope with a simple
% name + extension, |article.cls|.
%    \begin{macrocode}
\typeout{^^J%
  Checking the filename parser^^J%
  ============================}
%    \end{macrocode}
%
%    \begin{macrocode}
\filename@parse{article.cls}
\def\reserved@a{article}
%    \end{macrocode}
%
%    \begin{macrocode}
\testtrue
\ifx\filename@base\reserved@a
  \ifx\filename@ext\@clsextension
  \else
    \testfalse
  \fi
\else
  \testfalse
\fi
\iftest
   \typeout{filename parser OK!}\pause
\else
  \typeout{^^J%
    The LaTeX2e installation has defined \noexpand\filename@parse.^^J%
    This appears to be incorrect.^^J%
    You should remove the incorrect definition from texsys.cfg^^J%
    and rebuild the format.}
  \errmessage{BAD LaTeX2e system!!}
  \expandafter\expandafter\expandafter\@@end
\fi
%
%    \end{macrocode}
%
% Check the input path by looking for |article.cls|. If |article.cls|
% is in the current directory it would be found anyway, so first check
% it is not there.
%    \begin{macrocode}
\typeout{^^J%
  Checking the input path^^J%
  =======================^^J}
%    \end{macrocode}
%
%    \begin{macrocode}
\begingroup
\let\input@path\@undefined
\ifx\@currdir\@empty\else
  \IfFileExists{\@currdir article.cls}
   {\typeout{%
      article.cls appears to be in current directory!^^J^^J%
      If this is the case, install article.cls into a^^J%
      `standard input directory'^^J%
      and copy ltxcheck.tex to another directory before^^J%
      processing with LaTeX.^^J%
      ^^J%
      If article.cls is not in the current directory,^^J%
      then you need to edit texsys.cfg.^^J%
      Read the comments in that file. If nothing else works, add:^^J%
      \string\let\string\@currdir\string\@empty^^J}%
    \errhelp{Move files, or edit texsys.cfg}
    \def\ArticleClassFoundInCurrentDirectory{%
      This file should not be run in a `standard input directory'}
    \errmessage{BAD: \ArticleClassFoundInCurrentDirectory}}
    {}
\fi
\endgroup
%    \end{macrocode}
%
%    \begin{macrocode}
\IfFileExists{article.cls}
  {\typeout{input path OK!}}
  {\typeout{^^J%
     LaTeX claims that article.cls is not on the system.^^J%
     Either LaTeX has been incorrectly installed, or the
     \noexpand\input@path^^J%
     is incorrect. A correct definition should be added to^^J%
     texsys.cfg, and the format remade.}
   \pause
   \typeout{^^J%
     Typical definitions of \noexpand\input@path include:^^J^^J%
     \string\let\string\input@path=\noexpand\@undefined
      (the default definition)^^J^^J%
     \string\def\string\input@path{\@percentchar^^J
       {/usr/lib/tex/inputs/} {/usr/local/lib/tex/inputs/} }^^J^^J%
     \string\def\string\input@path{\@percentchar^^J
       {c:/tex/inputs/} {a:/} }^^J^^J%
     \string\def\string\input@path{\@percentchar^^J
       {tex_inputs:} {SOMEDISK:[SOMEWHERE.TEX.INPUTS]} }^^J}%
   \pause
   \typeout{^^J%
     Note that \noexpand\input@path should be undefined
       unless your^^J%
     TeX installation does not make
       \noexpand\openin and \noexpand\input^^J%
     search the same directories.^^J%
     If \noexpand\input@path is defined, entries should be^^J%
     in the same syntax as \noexpand\@currdir^^J%
     ie full directory names that may be concatenated with the^^J%
     basename (note the final / and ] in the above examples).^^J%
     Some systems may need more complicated settings.^^J%
     See texsys.cfg for more examples.^^J%
    ! BAD \noexpand\input@path!!}
   \@@end}%
\pause
%    \end{macrocode}
%
% For versions prior to \TeX3 complain to the installer. (Although
% \LaTeX\ will work with these old \TeX\ versions).
% For versions between 3 and 3.14 check that \LaTeX\ is using the
% work-around for the |^^J| in |\message| bug.
%    \begin{macrocode}
\typeout{^^J%
  Checking the TeX version^^J%
  ========================}
%    \end{macrocode}
%
% \changes{v0.2j}{1994/02/25}
%         {\cs{noboundary} is \cs{relax} not undef in TeX2 (initialised
%         in 2e format)}
%    \begin{macrocode}
\dimen@\ifx\@TeXversion\@undefined4\else\@TeXversion\fi\p@%
\ifx\noboundary\relax
  \typeout{^^J%
    This is TeX 2. You will not be able to use all the new features^^J%
    of LaTeX2e with such an old TeX.^^J%
    The current version (1995/12/11) is TeX 3.14159.^^J%
    Consider upgrading your TeX.}
  \ifdim\dimen@<3\p@\else
     \errhelp{Check that texsys.cfg has not defined \@TeXversion}
     \def\OldTeX{%
       BAD: \noexpand\@TeXversion is incorrect: \meaning\@TeXversion}
     \errmessage{\OldTeX}
  \fi
\else
%    \end{macrocode}
%
% \changes{v1.0h}{1994/10/11}
%         {Check for TeX3.141}
%    \begin{macrocode}
    \ifdim\dimen@>3.14\p@
      \typeout{This appears to be a recent version of TeX!^^J%
       If the following `lines' all appear on the same line,^^J%
       separated by \string^\string^J %
       then there has been an incorrect installation.}
    \else
      \typeout{^^J%
       This appears to be a TeX between 3.0 and 3.14^^J%
       but the current version (1995/12/11) is TeX 3.14159^^J%
       consider upgrading your TeX.^^J%
       The following `lines' will appear on the same line,^^J%
       separated by \string^\string^J;^^J%
       the same problem may affect other messages from LaTeX.}
     \fi
%    \end{macrocode}
%
%    \begin{macrocode}
\message{line1^^Jline2^^Jline3}
\pause
%    \end{macrocode}
%
%    \begin{macrocode}
\fi
%    \end{macrocode}
%
%
% To check that the \LaTeX\ fonts have been installed, the well known
% trick of going into |\batchmode|, and testing for |\nullfont| is used.
% Not all fonts are tested, just a representative sample.
%    \begin{macrocode}
\typeout{^^J%
  Checking fonts^^J%
  =====================================}
%    \end{macrocode}
% \changes{v1.0h}{1994/10/11}
%         {Check for fonts}
%    \begin{macrocode}
\def\checkfont#1{%
  \batchmode
  \font\test=#1\relax
  \errorstopmode
  \ifx\test\nullfont
    \typeout{\@spaces! BAD: #1.tfm not found!}
    \@tempswatrue
  \else
    \typeout{\@spaces OK: #1.tfm found}
  \fi}
%    \end{macrocode}
%
%    \begin{macrocode}
\typeout{^^JChecking Standard TeX fonts...}
\@tempswafalse
\checkfont{cmr10}
\checkfont{cmr12}
\checkfont{cmmi10}
\if@tempswa
  \errhelp{Obtain a complete standard TeX font distribution.}
  \errmessage{BAD: Missing Standard Fonts}
\else
%    \end{macrocode}
% \changes{v1.0s}{1996/07/19}
%         {Check for bad cm fonts}
%    \begin{macrocode}
    \font\testcm=cmr10
    \testcm
    \setbox0\hbox{h{}o}
    \setbox2=\hbox{ho}
    \ifdim\wd0=\wd2
     \typeout{^^J%
OK: correct Computer Modern fonts installed.}%
    \else
     \typeout{^^J%
An unauthorised and incompatible release of the^^J%
Computer Modern fonts has been installed on your system.^^J%
The official fonts may be obtained from CTAN archives in:^^J%
ctan:fonts/cm^^J%
For further details see Donald Knuth's Home page:^^J%
http://www-cs-faculty.stanford.edu/\protect~knuth/cm.html}%
  \errhelp{Re-install Computer Modern fonts, and then rebuild LaTeX}
  \errmessage{BAD Standard fonts!!}
    \fi
%    \end{macrocode}
%
%    \begin{macrocode}
  \pause
\fi
%    \end{macrocode}
%
%    \begin{macrocode}
\typeout{^^JChecking LaTeX Picture Mode fonts...}
\@tempswafalse
\checkfont{lcircle10}
\checkfont{lcirclew10}
\if@tempswa
  \@tempswafalse
  \checkfont{circle10}
  \checkfont{circlew10}
  \if@tempswa
    \typeout{^^J! BAD: You do not have the picture mode fonts:^^J%
           lcircle10 and lcirclew10}
  \else
    \typeout{^^J! BAD:%
           You have the picture mode fonts with their old names:^^J%
           circle10 and circlew10 have been renamed to^^J%
           lcircle10 and lcirclew10}
  \fi
  \errhelp{Obtain a complete standard LaTeX font distribution.}
  \errmessage{BAD: Missing LaTeX Fonts}
\else
  \pause
\fi
%    \end{macrocode}
%
%    \begin{macrocode}
\typeout{^^JChecking Extra LaTeX Computer Modern fonts...}
\@tempswafalse
\checkfont{cmmib5}
\checkfont{cmmib7}
\checkfont{cmex7}
\if@tempswa
\typeout{! BAD:^^J%
 LaTeX2e uses a few `extra' Computer Modern fonts produced by^^J%
 The American Mathematical Society.^^J%
 If you install The AMSFONTS font collection, then these, and other,^^J%
 fonts will be available to LaTeX.^^J%
 Although installing AMSFONTS is recommended, LaTeX does not require^^J%
 The full collection; you may obtain a minimal set of extra LaTeX^^J%
 fonts from any CTAN archive, in: ctan:macros/latex/fonts/}
\errhelp{Obtain LaTeX fonts or  the AMSFONTS collection.}
\errmessage{BAD: Missing LaTeX Fonts}
\else
  \pause
\fi
%    \end{macrocode}
%
% \changes{v1.0k}{1995/09/27}
%         {Check for dc and tc fonts}
% \changes{v1.1a}{1997/01/14}
%         {Check for ec fonts}
% \changes{v1.1c}{1997/06/10}
%         {Modify messages now ec released}
%    \begin{macrocode}
\typeout{^^JChecking T1 encoded Computer Modern (dc & ec) fonts...}
%    \end{macrocode}
% \changes{v1.0m}{1995/10/31}
%         {Check the T1 fd files match the  dc release.}
% This command looks for the string |dcr17<| in the font tables for
% T1/cmr. If it is there, then the T1 fd files match the old dc fonts,
% for dc release 1.1 or earlier. If not then presumably new fd files
% are being used.
%    \begin{macrocode}
\def\dcrseventeen{%
  \begingroup
    \escapechar-1
    \xdef\reserved@a{%
      \noexpand\in@
        {\expandafter\string\csname dcr17\endcsname<}%
        {\expandafter\expandafter\expandafter
           \string\csname T1/cmr/m/n\endcsname<}}%
  \endgroup
  \reserved@a}
%    \end{macrocode}
% Similarly this command looks for the string |ecrm| in the font tables
% for T1/cmr. If it is there, then the T1 fd files match the ec fonts,
% for ec release 1.0 or later.
%    \begin{macrocode}
\def\ecrm{%
  \begingroup
    \escapechar-1
    \xdef\reserved@a{%
      \noexpand\in@
        {\expandafter\string\csname ecrm\endcsname}%
        {\expandafter\expandafter\expandafter
           \string\csname T1/cmr/m/n\endcsname}}%
  \endgroup
  \reserved@a}
%    \end{macrocode}
% \changes{v1.0o}{1995/11/14}
%    {dont produce a BAD message if just one set of dc fonts is missing}
% Remove the ``! BAD'' typeout while checking for dc fonts so
% as not to worry sites with just the new ones.
%    \begin{macrocode}
\def\checkfont#1{%
  \batchmode
  \font\test=#1\relax
  \errorstopmode
  \ifx\test\nullfont
    \typeout{\@spaces\@spaces #1.tfm not found}
    \@tempswatrue
  \else
    \typeout{\@spaces OK: #1.tfm found}
  \fi}
%    \end{macrocode}
%

%    \begin{macrocode}
\@tempswafalse
\checkfont{ecrm1000}
\if@tempswa
%    \end{macrocode}
% No ec fonts. Check the state of the dc fonts.
%
%    \begin{macrocode}
\typeout{No EC fonts found, checking DC fonts...}
\@tempswafalse
\checkfont{dcr10}
\if@tempswa
  \@tempswafalse
  \checkfont{tcr1000}
  \if@tempswa
%    \end{macrocode}
% No dc fonts at all.
%    \begin{macrocode}
    \typeout{^^J%
! BAD: No ec fonts found!!^^J%
LaTeX does not require the use of ec fonts^^J%
however they are strongly recommended.^^J%
The ec fonts are available in a more natural range of sizes^^J%
and allow better hyphenation and kerning than the^^J%
old fonts such as cmr10.^^J%
These ec fonts may be obtained from CTAN archives, in:^^J%
ctan:fonts/ec}
  \else
%    \end{macrocode}
% No old dc fonts, but new ones installed.
% First check whether the latest patch has been applied.
% \changes{v1.0p}{1995/12/11}
%         {Check for dc fonts 1.2 patch level 1 (Bernd Raichle) /2003}
% \changes{v1.0q}{1996/06/03}
%         {Check for dc fonts 1.3}
% \changes{v1.1b}{1997/01/24}
%         {extra closing brace removed from this branch}
%    \begin{macrocode}
    \font\testdc=dcr1000
    \testdc
    \setbox0\hbox{A{}y}
    \setbox2=\hbox{Ay}
    \ifdim\wd0>\wd2
     \typeout{^^J%
! BAD: dc fonts release 1.3 installed^^J%
The dc fonts are now replaced by the ec fonts^^J%
These ec fonts may be obtained from CTAN archives, in:^^J%
ctan:fonts/ec.}%
    \else
     \typeout{^^J%
! BAD dc fonts 1.2 or older installed.^^J%
The dc fonts are now replaced by the ec fonts^^J%
These ec fonts may be obtained from CTAN archives, in:^^J%
ctan:fonts/ec.}%
    \fi
    \dcrseventeen
    \ifin@
      \typeout{^^J%
The fd files for the obsolete release 1.1 of the^^J%
dc fonts have been loaded into the LaTeX format.^^J%
However, you appear to have at least release 1.2 of the dc fonts.^^J%
You should generate suitable fd files by running:^^J%
latex newdc.ins^^J%
and then rebuild the format by rerunning:^^J%
initex latex.ltx}
       \errmessage{BAD LaTeX2e system!!}
     \else
       \typeout{^^J%
         DC fonts OK!}
    \fi
  \fi
\else
  \@tempswafalse
  \checkfont{tcr1000}
  \if@tempswa
%    \end{macrocode}
% Old DC fonts, but no new ones.
%    \begin{macrocode}
    \typeout{^^J%
Old dc fonts found!!^^J%
Only the original dc fonts are on your system.^^J%
Later releases of the dc/ec fonts introduced^^J%
many improvements and are strongly recommended.^^J%
They may be obtained from CTAN archives, in:^^J%
ctan:fonts/ec.}
    \pause
    \dcrseventeen
    \ifin@\else
      \typeout{^^J%
The LaTeX2e installation has installed fd files for^^J%
release 1.2 (or later) of the dc fonts.^^J%
However, you appear to have only release 1.1 of these fonts.^^J%
You must now generate the correct fd files by running:^^J%
latex olddc.ins^^J%
and then rebuild the format by rerunning:^^J%
initex latex.ltx}
      \errmessage{BAD LaTeX2e system!!}
    \fi
  \else
%    \end{macrocode}
% Both old and new DC fonts.
%    \begin{macrocode}
    \font\testdc=dcr1000
    \testdc
    \setbox0\hbox{A{}y}
    \setbox2=\hbox{Ay}
    \ifdim\wd0>\wd2
     \typeout{^^J%
! BAD: dc fonts release 1.3 installed^^J%
The dc fonts are now replaced by the ec fonts^^J%
These ec fonts may be obtained from CTAN archives, in:^^J%
ctan:fonts/ec.}%
    \else
     \typeout{^^J%
! BAD dc fonts 1.2 or older installed.^^J%
The dc fonts are now replaced by the ec fonts^^J%
These ec fonts may be obtained from CTAN archives, in:^^J%
ctan:fonts/ec.}%
    \fi
%    \end{macrocode}
%
%    \begin{macrocode}
    \dcrseventeen
    \ifin@
      \typeout{^^J%
The fd files for the obsolete release 1.1 of the^^J%
dc fonts have been loaded into the LaTeX format.^^J%
However, you appear to have at least release 1.2 of the dcfonts.^^J%
You should use generate suitable fd files by running:^^J%
latex newdc.ins^^J%
and then rebuild the format by running:^^J%
initex latex.ltx^^J%
Otherwise LaTeX will always use the older fonts.}
       \errmessage{BAD LaTeX2e system!!}
    \else
      \ecrm
      \ifin@
        \typeout{^^J%
The fd files for the new EC fonts have been loaded into^^J%
the LaTeX format.^^J%
However, these fonts are not found by LaTeX.^^J%
You should either install the ec fonts, or generate suitable^^J%
fd files for the dc fonts by running: \space latex newdc.ins^^J%
and then rebuild the format by running: \space initex latex.ltx}
       \errmessage{BAD LaTeX2e system!!}
      \else
        \typeout{^^J%
DC fonts OK!^^J%
(Both old and new dc font releases are installed.)^^J%
Note that the dc fonts are expected to be replaced by ec^^J%
in January 1997.}
      \fi
    \fi
  \fi
\fi
%    \end{macrocode}
% Else EC fonts are found, so check whether LaTeX is going to use them.
%
%    \begin{macrocode}
\else
%    \end{macrocode}
%
%    \begin{macrocode}
  \ecrm
  \ifin@
   \typeout{EC fonts OK!}
  \else
    \typeout{%
EC fonts installed but LaTeX is still using dc fonts.^^J%
You may want to run ec.ins and remake the LaTeX format}
  \fi
%    \end{macrocode}
%
%    \begin{macrocode}
\fi
\pause
%    \end{macrocode}
%
%
%
% The following files will be unpacked by running iniTeX on
% |unpack.ins|.
%
%    \begin{macrocode}
\typeout{^^JChecking LaTeX input files...^^J}
%    \end{macrocode}
%
% If the specified file is not there, add it to the list.
%    \begin{macrocode}
\def\checkfile#1{%
  \IfFileExists{#1}{}{\edef\missingfile{\missingfile#1, }}}
%    \end{macrocode}
%
% Report any missing files in the last batch tested.
%    \begin{macrocode}
\def\filereport#1#2{%
\ifx\missingfile\@empty
 \typeout{^^J%
OK: The #1 files such as #2^^J%
are accessible to LaTeX.}
\pause
\expandafter\@gobbletwo
\else
  \typeout{^^J%
! BAD: The #1 files:^^J%
\missingfile^^J%
are not accessible to LaTeX.}
\errhelp{Check the installation!}
\let\missingfile\@empty
\fi
\errmessage{Missing LaTeX files}}
%    \end{macrocode}
%
% Kernel files:
%    \begin{macrocode}
\let\missingfile\@empty
%    \end{macrocode}
%
%    \begin{macrocode}
\checkfile{hyphen.ltx}
\checkfile{fontmath.ltx}
\checkfile{fonttext.ltx}
\checkfile{preload.ltx}
\checkfile{texsys.cfg}
\checkfile{latex.ltx}
%    \end{macrocode}
%
% Don't use |\filereport| here as the message is rather different
% as the |.ltx| files don't really need to be available to \LaTeX\
% once the format is made.
%    \begin{macrocode}
\ifx\missingfile\@empty
 \typeout{^^J%
OK: The files such as latex.ltx that are used to make^^J%
the format are  accessible to LaTeX.}
\else
  \typeout{^^J%
The files:^^J%
\missingfile^^J%
that are used to make the format are not accessible to LaTeX.^^J%
This is OK, but you will need those files if you need to remake the^^J%
the format later.}
\fi
\pause
\let\missingfile\@empty
%    \end{macrocode}
%
% Class files and class options:
%    \begin{macrocode}}
\checkfile{article.cls}
\checkfile{report.cls}
\checkfile{book.cls}
\checkfile{letter.cls}
\checkfile{ltxdoc.cls}
\checkfile{proc.cls}
\checkfile{slides.cls}
\checkfile{bk10.clo}
\checkfile{bk11.clo}
\checkfile{bk12.clo}
\checkfile{size10.clo}
\checkfile{size11.clo}
\checkfile{size12.clo}
\checkfile{fleqn.clo}
\checkfile{leqno.clo}
%    \end{macrocode}
%
%    \begin{macrocode}
\filereport{main class}{article.cls}
%    \end{macrocode}
%
% Package files:
%    \begin{macrocode}
\checkfile{alltt.sty}
\checkfile{doc.sty}
\checkfile{exscale.sty}
\checkfile{flafter.sty}
\checkfile{fontenc.sty}
\checkfile{graphpap.sty}
\checkfile{ifthen.sty}
\checkfile{inputenc.sty}
\checkfile{latexsym.sty}
\checkfile{makeidx.sty}
\checkfile{newlfont.sty}
\checkfile{oldlfont.sty}
\checkfile{shortvrb.sty}
\checkfile{showidx.sty}
\checkfile{slides.sty}
\checkfile{syntonly.sty}
\checkfile{tracefnt.sty}
%    \end{macrocode}
%
%
%    \begin{macrocode}
\filereport{main package}{ifthen.sty}
%    \end{macrocode}
%
% Font definition (.fd) files:
%    \begin{macrocode}}
\checkfile{omlcmm.fd}
\checkfile{omlcmr.fd}
\checkfile{omllcmm.fd}
\checkfile{omscmr.fd}
\checkfile{omscmsy.fd}
\checkfile{omslcmsy.fd}
\checkfile{omxcmex.fd}
\checkfile{omxlcmex.fd}
\checkfile{ot1cmdh.fd}
\checkfile{ot1cmfib.fd}
\checkfile{ot1cmfr.fd}
\checkfile{ot1cmr.fd}
\checkfile{ot1cmss.fd}
\checkfile{ot1cmtt.fd}
\checkfile{ot1cmvtt.fd}
\checkfile{ot1lcmss.fd}
\checkfile{ot1lcmtt.fd}
\checkfile{t1cmdh.fd}
\checkfile{t1cmfib.fd}
\checkfile{t1cmfr.fd}
\checkfile{t1cmr.fd}
\checkfile{t1cmss.fd}
\checkfile{t1cmtt.fd}
\checkfile{t1cmvtt.fd}
\checkfile{ts1cmr.fd}
\checkfile{ts1cmss.fd}
\checkfile{ts1cmtt.fd}
\checkfile{ts1cmvtt.fd}
\checkfile{ucmr.fd}
\checkfile{ucmss.fd}
\checkfile{ucmtt.fd}
\checkfile{ullasy.fd}
\checkfile{ulasy.fd}
%    \end{macrocode}
%
%
%    \begin{macrocode}
\filereport{font definition}{t1cmr.fd}
%    \end{macrocode}
%
% Font encoding files:
%    \begin{macrocode}
\checkfile{t1enc.def}
\checkfile{ot1enc.def}
\checkfile{omsenc.def}
\checkfile{omlenc.def}
%    \end{macrocode}
%
%
%    \begin{macrocode}
\filereport{font encoding}{t1enc.def}
%    \end{macrocode}
%
% Input encoding files:
%    \begin{macrocode}
\checkfile{ascii.def}
\checkfile{latin1.def}
\checkfile{latin2.def}
\checkfile{latin3.def}
\checkfile{latin5.def}
\checkfile{cp850.def}
\checkfile{cp852.def}
\checkfile{cp865.def}
\checkfile{cp437.def}
\checkfile{cp437de.def}
\checkfile{applemac.def}
\checkfile{next.def}
\checkfile{ansinew.def}
%    \end{macrocode}
%
%    \begin{macrocode}
\filereport{input encoding}{latin1.def}
%    \end{macrocode}
%
% Compatibility files:
%    \begin{macrocode}
\checkfile{article.sty}
\checkfile{book.sty}
\checkfile{letter.sty}
\checkfile{proc.sty}
\checkfile{report.sty}
\checkfile{fleqn.sty}
\checkfile{leqno.sty}
\checkfile{openbib.sty}
\checkfile{latex209.def}
%    \end{macrocode}
%
%
%    \begin{macrocode}
\filereport{compatibility mode}{article.sty}
%    \end{macrocode}
%
% Other files:
%    \begin{macrocode}
\checkfile{bezier.sty}
\checkfile{docstrip.tex}
\checkfile{slides.def}
\checkfile{sfonts.def}
\checkfile{t1enc.sty}
%    \end{macrocode}
%
%    \begin{macrocode}
\filereport{remaining}{sfonts.def}
%    \end{macrocode}
%
%    \begin{macrocode}
\@@end
%    \end{macrocode}
%
% \Finale
%


==> caption/CHANGELOG <==
Changes made in the caption package bundle
==========================================

Please note that this document does not reflect bugfix-releases (which are marked with a letter after the version number, for example v3.4m), and that the dates given are the dates of the release w/o bugfixes.

If you are interested in a complete changelog -- including bugfixes -- process the dtx files with \RecordChanges and \PrintChanges.


caption package
---------------

v1.0 (1994/10/27)
- 1st published version

v1.1 (1994/11/03)
- New option `centerlast'

v1.2 (1994/11/28)
- Support of the `float' package added

v1.3 (1995/01/09)
- Support of \captionlabelfont in subcaptions added

v1.4 (1995/01/30)
- New option `nooneline'

v2.0 (caption2, 1995/10/09)
- New experimental version with many new commands and features
- Support of the `longtable' package added

v2.1 (caption2, 2002/02/26)
- Adapted to version 2.1 of the subfigure package
- New options for interaction with other packages (float,...)
- New command \normalcaptionparams
- New commands \captionof and \captionof*
- New ifs \ifcaptionlabel and \ifignoreLTcapwidth
- \realcaptionwidth renamed to \captionlinewidth

v2.2 (caption2, 2007/04/06)
- Internal change: Uses the caption3 kernel now

v3.0 (2003/12/20)
- Completely rewritten in cooperation with Frank Mittelbach and Steven Cochran

v3.1 (2007/09/01)
- Improved compatibility to supported document classes and packages, but decreased compatibility to non-supported document classes and packages
- Support of the AMS & SMF document classes added
- Support of the `beamer' document class added
- Support of the `KOMA-Script' document classes added
- Support of the `floatflt' package added
- Support of the `fltpage' package added
- Support of the `picinpar' package added
- Support of the `picins' package added
- Support of the `threeparttable' package added
- Support of the `wrapfig' package added
- Support of the `xtab' package added
- Check against incompatible `ftcap' package added
- Check against incompatible `nonfloat' package added
- Check against incompatible `topcapt' package added
- Does not process global options anymore to avoid conflicts with document class options
- New option compatibility=
- New options font+=, labelfont+= & textfont+=
- New options hypcap= & hypcapspace=
- New options list= and listformat=
- New option options=
- New options figurewithin= and tablewithin=
- Starred variant of option margin*= added
- Starred variant of option style*= added
- Starred variant of option type*= added
- Font options `normal', `normalcolor', `color', `normalfont' & `stretch' added
- Default position changed from `bottom' to `auto'
- New command \DeclareFloatingEnvironment resp. \DeclareCaptionType
- New command \DeclareCaptionListFormat
- New command \captionlistentry
- Starred variant of \clearcaptionsetup added
- Optional argument added to \clearcaptionsetup
- Starred variant of \ContinuedFloat added
- \captionsetup{...} inside longtables added
- \captionsetup[singleline]{...} added
- A \label before \caption will result in warning "\label before \caption ignored"
- The counters lofdepth & lotdepth are supported now
- Label formats have three arguments now
- Optional argument added to \DeclareCaptionFormat; "format=plain" removed from single-line options of default format
- Caption label format `brace' added

v3.2 (2011/07/30)
- Support of `beamer' document class improved
- Support of `magyar' babel option added
- Support of `sansmath' package added
- Support of `titletoc' package added to \DeclareCaptionType & \DeclareCaptionSubType
- Support of `tocbasic' package added to \DeclareCaptionType
- New options calcmargin=, calcmargin*=, calcwidth=, and calcwidth*=
- New option listtype= added
- New option parboxrestore=partial/full
- New options within= & without
- Option slc= as abbreviation of singlelinecheck= added
- Pre-defined text format `empty' added
- New command \captionbox
- New command \phantomcaption
- New command \setcaptiontype as replacement for \captionsetup{type=...}
- New command \setcaptionsubtype as replacement for \captionsetup{subtype}
- "Hyperref support is turned off because hyperref has stopped early" is not a warning anymore but an information instead

v3.3 (2013/01/06)
- Revised handling of continued floats and sub-captions
- New option box= and appropriate command \DeclareCaptionBox
- New option list-entry= (see also endfloat package documentation)
- Support of multiple optional arguments added to \captionsetup (see bicaption package documentation)
- Adapted to the elsarticle document class
- Adapted to the current version of memhfixc package, provided by the memoir document class
- Fixed compatibility problem with breqn and nag packages
- Corrects incorrect load order hyperref-float now (needs hyperref v6.82q or newer)
- New switch \ifsinglelinecaption for usage inside own commands added

v3.4 (2019/09/11)
- Label format `autodot' added (for usage within documents using KOMA-Script document class)
- Label format `unnumbered' added
- \ContinuedFloat renamed to \continuedfloat (since this is not a preamble command)
- \caption will always be re-defined now, unless `compatibility' is set to `v1' (or an incompatible package is loaded)

v3.5 (2020/08/30)
- If a document class defines \caption@documentclass, an adaption to the caption package will be loaded as caption-<documentclass>.sto
- New commands \SetCaptionDefault, \AtCaptionPackage, and \AfterCaptionPackage for usage in document classes or document class adaptions
- Document class support re-written (using the new commands above)
- New commands \caption@switchdefault and \caption@restoredefault for usage in babel language packages
- Babel language support re-written (using the new commands above); furthermore it's independent on the load order now
- Support for the babel language option `latvian' added
- New command \DeclareCaptionSinglelinecheck
- New commands \ForEachCaptionType and \ForEachCaptionSubType
- Options "figure*" resp. "table*" will be applied additionally in "figure*" resp. "table*" environments (twocolumn mode only)
- Option and font option "hypersetup" added which expands to \hypersetup (if defined) resp. nothing (otherwise)


bicaption package
-----------------

v0.9 (2010/09/19)
- 1st published version (see also http://www.mrunix.de/forums/showthread.php?t=68312)

v1.0 (2011/09/03)
- Support for list entries added

v1.1 (2012/12/26)
- \captionmainlanguage and \selectcaptionlanguage added

v1.2 (2016/03/27)
- \DeclareLangDependantCaptionOption added

v1.3 (2020/10/25)
- Option "bi-separator" and command \DeclareBiCaptionSeparator added


ltcaption package
-----------------

v1.0 (2007/04/15)
- 1st version

v1.1 (2007/09/01)
- Adapted to the NTG document classes (Support of \CaptionLabelFont & \CaptionTextFont added)
- Adapted to the `floatrow' package by Olga Lapko
- New macro \LTcaptype
- New environment longtable*

v1.2 (2008/03/28)
- New skip \LTcapskip

v1.3 (2011/09/12)
- New macro \CaptionLabelSeparator

v1.4 (2013/06/01)
- Adapted to the memoir document class (v3.7b)


subcaption package
------------------

v1.0 (2008/03/16)
- 1st published version

v1.1 (2011/08/17)
- New caption option subrefformat=
- New command \phantomsubcaption

v1.2 (2018/05/13)
- Values `B' and `T' for the optional argument <outer-pos> added to the environments `subfigure' and `subtable'

v1.3 (2019/08/31)
- New command \subfloat for easy transition from the `subfig' package


==> caption/README <==
==========================================================================

The `caption' package bundle
Release 2020-10-26
Copyright (C) 1994-2020 Axel Sommerfeldt (axel.sommerfeldt@f-m.fm)

License: LPPL = LaTeX Project Public Licence
Maintenance Status: maintained (by Axel Sommerfeldt)

Home page:
  https://gitlab.com/axelsommerfeldt/caption

If you need help for installation please visit:
  https://texfaq.org/FAQ-inst-miktexstar
  https://texfaq.org/FAQ-installthings
  https://texfaq.org/FAQ-privinst

If you need help using these packages please visit:
  https://latex.org/forum/
  https://tex.stackexchange.com/
  https://golatex.de/               (German)
  https://texwelt.de/               (German)

If you think you may have found a bug in these packages,
or want to report a suggestion for improvement, please either visit
  https://gitlab.com/axelsommerfeldt/caption/issues
or send an e-mail to
  axel.sommerfeldt@f-m.fm

--------------------------------------------------------------------------

The `caption' package v3.5 offers customization of captions of floating
environments such `figure' and `table' and cooperates with the packages

  float, floatflt, fltpage, hyperref, hypcap, listings, longtable,
  picinpar, picins, rotating, sidecap, subfigure, supertabular,
  threeparttable, wrapfig, and xtab.

Furthermore the `floatrow', the `subcaption', and the `subfig' package
supports the `caption' package and uses its \captionsetup interface.

User Manual: caption-eng.pdf (English)
             caption-rus.pdf (Russian, outdated)
             caption-deu.pdf (German)

--------------------------------------------------------------------------

The `bicaption' package v1.3 is a tiny package supporting the typesetting
of bilingual captions.

User Manual: bicaption.pdf (English)

--------------------------------------------------------------------------

The `ltcaption' package v1.4 fixes caption problems with
other-than-center aligned longtables. (solving LaTeX PR `tools/3387')

A bonus feature is the addition of the environment longtable* which does
not increment the table counter.

This package will be loaded automatically by the `caption' package,
but can be used without the caption package, too.

User Manual: ltcaption.pdf (English)

--------------------------------------------------------------------------

The `subcaption' package v1.3 is a small package supporting typesetting
of sub-captions (by using the the sub-caption feature of the `caption'
package).

User Manual: subcaption.pdf (English)

--------------------------------------------------------------------------

Note: The `newfloat' package was removed from this package bundle and was
uploaded to CTAN as stand-alone package.

Note: The `totalcount' package was removed from this package bundle and
was uploaded to CTAN as stand-alone package.

==========================================================================
(The pictures cat.eps & elephant.eps were taken with permission from the
 LaTeX Companion examples.)


==> hyperref/abbr.tex <==
\abbrdef{``}{\texorpdfstring{``}{\flqq}}
\abbrdef{''}{\texorpdfstring{''}{\frqq}}
\abbrdef{acroread}{\Program{AcrobatReader}}
\abbrdef{aux}{\File{.aux}}
\abbrdef{eg}{e.\,g\mbox{.}}
\abbrdef{gdi}{general document information}
\abbrdef{gs}{\Program{ghost\-script}}
\abbrdef{hyperref}{\Package{hy\-per\-ref}}
\abbrdef{hypbmsec}{\Package{hypbmsec}}
\abbrdef{ind}{\hbox{\texttt{ \ }}}
\abbrdef{isolatin1}{ISOLatin1}
\abbrdef{latex}{\LaTeX}
\abbrdef{latexe}{\texorpdfstring{\LaTeXe}{LaTeX2e}}
\abbrdef{mediabox}{/MediaBox}
\abbrdef{PD1}{PD1}
\abbrdef{pdf}{PDF}
\abbrdef{pdfdocencoding}{PDFDocEncoding}
\abbrdef{pdffile}{pdf file}
\abbrdef{pdfinfo}{\Program{pdfinfo}}
\abbrdef{pdfspec}{*pdf* specification}
\abbrdef{pdfstringdef}{\cms{pdfstringdef}}
\abbrdef{pdftex}{\Program{\pdfTeX}}
\abbrdef{perlscript}{perl script}
\abbrdef{plain}{plain}
\abbrdef{plaintex}{*plain*-*tex*}
\abbrdef{postscript}{PostScript}
\abbrdef{PU}{PU}
\abbrdef{sectioning}{section} % section?
\abbrdef{Sectioning}{Section}
\abbrdef{tex}{\TeX}
\abbrdef{texfile}{*tex* file}
\abbrdef{thumbpdf}{\Package{thumb\-pdf}}
\abbrdef{thumbpdf.pl}{\File{thumbpdf.pl}}
\abbrdef{toc}{\File{.toc}}
\abbrdef{unicode}{Unicode}
\abbrdef{winansiencoding}{WinAnsiEncoding}
\endinput


==> hyperref/docinfo.tex <==
\foilhead[-\baselineskip]{General Document Information}

%\begin{Nav}{\NavInfo\NavBack}%
\begin{Nav}{\NavInfo}%
  \newcommand{\tit}[1]{%
    \multicolumn{2}{@{}l@{}}{\textbf{#1}}\\[0.5ex]%
  }
  \newcommand{\longentry}[1]{%
    \multicolumn{2}{@{}l@{}}{#1}%
  }
  \noindent
  Application: search engines.

  \noindent
  \begin{minipage}[t]{.55\linewidth}
    \begin{tabular}[t]{@{}l>{\tt}l@{}}
    \tit{\hypertarget{info}{*hyperref* options:}}%
    Title:&\Blue{pdftitle}\\
    Subject:&\Blue{pdfsubject}\\
    Author:&\Blue{pdfauthor}\\
    Keywords:&\Blue{pdfkeywords}\\
    Creator:&\Blue{pdfcreator}\\
    Producer:&\Blue{pdfproducer}
    \end{tabular}
  \end{minipage}%
  \begin{minipage}[t]{.45\linewidth}
    \begin{tabular}[t]{@{}ll@{}}
      \tit{Times:}%
      Created:&\Green{/CreationDate}\\
      Modificated:&\Green{/ModDate}\\[1ex]
      \tit{Informations:}%
      \longentry{File name, file size}\\
      \longentry{*pdf* version}\\
      \longentry{Optimized(linearized)}
    \end{tabular}
  \end{minipage}

  \subfoilhead{Setting\texorpdfstring{ the general document information}{}}
  \begin{smallpar}\hypertarget{infoanw}{}%
  \noindent
  \Code{\cms{usepackage}\{hyperref\}}\par
  \vspace{-\parskip}
  \catcode`\^^M=5
  \verbatiminput{pdfinfo}
  \end{smallpar}
  \newpage

\end{Nav}


\iffalse
\begingroup
  \makeatletter
  \def\hyper@anchorstart#1\hyper@anchorend{}%
  \pdfbookmark[1]{\file{hyperref} options}{optinfo}
\endgroup
\fi

\endinput


==> hyperref/encoding.tex <==
\clearpage
\pdfbookmark[0]{Encodings}{enc}

\begingroup
\hypersetup{bookmarksopenlevel=2}


\subfoilhead[-\baselineskip]{Font encoding mechanism%
  \texorpdfstring{}{ of \abbr{latexe}}}

\noindent
\begin{tabular}{@{}l@{ }l@{ $\Rightarrow$ }l@{}}
plain-\TeX:& \code[green]<\ss>\ = \code[blue]<\char"19>&\Red{\ss}\\[1ex]
\LaTeXe:
  & \code<\fontencoding{OT1}\selectfont\char"19>&\Red{\ss}\\
  & \code<\fontencoding {T1}\selectfont\char"19>&\Red{\i}\\[0.5ex]
  & \code<\ss>\ = \code[blue]<\OT1-cmd \ss > \code[green]<\OT1\ss>&\Red{\ss}
\end{tabular}

\noindent
The font slot positions depend on the encoding:\\
\phantom{plain-\TeX: }\code[green]<\OT1\ss>\ = \code<\char"19>\\
\phantom{plain-\TeX: }\code[green]<\T1\ss>\phantom{\code<O>} =
  \code<\char"FF>\\
\phantom{plain-\TeX: }\code[green]<\?\ss>\phantom{\code<OT>} =
  \code<\UseTextSymbol{OT1}\ss>

%\begin{smallpar}
  \noindent
  \code<\> \code[blue]<OT1\ss>\ =
  \code<\csname > \code[blue]<OT1> \code<\string> \code[blue]<\ss>
    \code<\endcsname>
%\end{smallpar}


\subfoilhead[-\baselineskip]{PD1 encoding%
  \texorpdfstring{ (\abbr{pdfdocencoding})}{}}

\begin{itemize}
\def\1{\code[red]}%
\def\2{\code[blue]}\def\3{\Blue}%
\def\4#1{\Green{#1}\,=\,}%
\def\5{\Green}
\item Most names: \1<\text>%
    \3{\textsl{\textless glyph name\textgreater}}\\
    Examples:\quad
  \begin{tabular}[t]{@{}c@{\,=\,}l@{,\quad}c@{\,=\,}l@{}}
    \5\textregistered&\1<\text>\2<registered>&
    \5\textasciitilde&\1<\text>\2<asciitilde>
  \end{tabular}
\item Traditional *tex* and *latex* names.\\
    Examples:\quad
    \4\AE\2<\AE>,\quad
    \4\ss\2<\ss>
\item Accented characters.\\
    Examples:\quad
    \4{\"U}\2<\"U>,\quad
    \4{\c c}\2<\c c>,\quad
    \4{\r A}\2<\r A>~($\Leftarrow$\,\1<\AA>)
\item Escape octal sequences are the result:
%  \2<\textmu>\ (\Green{$\mu$}) $\Rightarrow$ \1<\265>
%  \2<\guillemotleft>\ (\Green{\guillemotleft}) $\Rightarrow$ \1<\253>
  \2<\textmu>\,$\Rightarrow$\,\1<\265>
\end{itemize}


\subfoilhead[-1.5\baselineskip]{PU encoding%
  \texorpdfstring{ (\abbr{unicode})}{}}

\begin{itemize}
\item[\frownie] Characters having catcodes 11 (letter) and 12 (other):\\
Checking each token, high memory and time consumption.
\item[\frownie] Ligatures: same as above.
\item[\frownie] Direct commands:\\
  Easier to implement, but each command must be redefined each time.
\item[\smiley] Commands of *latexe*'s fontencoding mechanism:\\
  Smallest memory consumption and fastest method.\\
  This method is used by package *hyperref*.
\end{itemize}


\subsubfoilhead[-\baselineskip]{Examples of \abbr{unicode} bookmarks}

\begingroup
\def\top#1{\vtop{\vskip0pt\hbox{#1}}}
\def\use#1{\top{\includegraphics[scale=1.2]{u0#1}}}
\centering
\begin{tabular}{@{}ll@{}}
\Blue{Greek}:&\Blue{Cyrillic}:\\
\use{3}&\use{4}\\
\end{tabular}
\par
\endgroup

\endgroup
\endinput


==> hyperref/ende.tex <==
\clearpage
\pdfbookmark[0]{Ende}{ende}

\subfoilhead[-1.5\baselineskip]{Zusammenfassung}
\begin{itemize}
  \item \Red{Dokumenteninformation}:
    \begin{itemize}
      \item \file{hyperref}-Optionen in \code[blue]<\hypersetup>.
    \end{itemize}
  \item \Red{Lesezeichen}:
    \begin{itemize}
      \item Vorsicht wegen fehlender Magenverarbeitung
      \item Vieles durch \code[blue]<hyperref.sty>\ automatisiert.
      \item Zusatzpaket \code[blue]<hypbmsec.sty>
      \item Besondere Effekte erfordern "`low level"'-Eingriffe.
    \end{itemize}
  \item \Red{Thumbnails}:
    \begin{itemize}
      \item
      Einfache Benutzerschnittstelle mit \code[blue]<thumbpdf>.
    \end{itemize}
\end{itemize}


\subfoilhead[-\baselineskip]{Bezugsquellen}

\begin{smallpar}
\pdfadjustspacing=1
\noindent
\begingroup
\def\it{\textbullet}%
\def\sep{1ex}%
\begin{tabularx}{\linewidth}{@{}l@{ }X@{}}
  \it&\Blue{PDF-Spezifikation}:\hfill
\url{http://www.adobe.com/supportservice/devrelations/PDFS/TN/PDFSPEC.PDF}\\[\sep]
  \it&\Blue{pdf\TeX}: \url{http://www.tug.org/applications/pdftex/}\\
  &Win32: \url{ftp://ftp.ese-metz.fr/pub/TeX/win32-beta/}\\
  &Dokumantation: \url{http://www.pragma-ade.nl/pdftex.htm}\\[\sep]
  \it&\Blue{hyperref}, \Blue{pd1enc.def}, \Blue{hyparen.sty}:
\url{ftp://ftp.dante.de/tex-archive/macros/latex/contrib/supported/hyperref/}\\[\sep]
  \it&\Blue{hypbmsec}: Noch per E-Mail, CTAN geplant.\\[\sep]
  \it&\Blue{thumbpdf}:\hfill
\url{ftp://ftp.dante.de/tex-archive/macros/pdftex/thumbpdf/}\\[\sep]
  \it&\Blue{ghostscript}:
\url{http://www.cs.wisc.edu/~ghost/} oder\\&
\url{http://ftp.dante.de/tex-archive/support/ghostscript/aladdin/}
\end{tabularx}
\endgroup
\end{smallpar}

\rightfooter{%
  \ifprint
  \else
    \NavFull\NavSep\NavPrev\NavSep\NavQuit
  \fi
}


==> hyperref/eurobm99.tex <==
%\includeonly{title,docinfo,strings,encoding,psd,hyperref,replace,pdfextra,thumb,summary,links,appendix}
%\includeonly{hyperref}

\begin{document}
\catcode`\*=\active
\include{title}
\include{docinfo}
\include{strings}
\include{encoding}
\include{psd}
\include{hyperref}
\include{replace}
\include{pdfextra}
\include{thumb}
\include{summary}
\include{links}
\include{appendix}
\end{document}


==> hyperref/fdl.tex <==
% This file is a chapter.  It must be included in a larger document to work
% properly.

\chapter{GNU Free Documentation License}

Version 1.2, November 2002


 Copyright \copyright\ 2000,2001,2002  Free Software Foundation, Inc.\\
     59 Temple Place, Suite 330, Boston, MA  02111-1307  USA\\
 Everyone is permitted to copy and distribute verbatim copies
 of this license document, but changing it is not allowed.


\section*{PREAMBLE}

The purpose of this License is to make a manual, textbook, or other
functional and useful document ``free'' in the sense of freedom: to
assure everyone the effective freedom to copy and redistribute it,
with or without modifying it, either commercially or noncommercially.
Secondarily, this License preserves for the author and publisher a way
to get credit for their work, while not being considered responsible
for modifications made by others.

This License is a kind of ``copyleft'', which means that derivative
works of the document must themselves be free in the same sense.  It
complements the GNU General Public License, which is a copyleft
license designed for free software.

We have designed this License in order to use it for manuals for free
software, because free software needs free documentation: a free
program should come with manuals providing the same freedoms that the
software does.  But this License is not limited to software manuals;
it can be used for any textual work, regardless of subject matter or
whether it is published as a printed book.  We recommend this License
principally for works whose purpose is instruction or reference.


\section{APPLICABILITY AND DEFINITIONS}
\label{applicability}

This License applies to any manual or other work, in any medium, that
contains a notice placed by the copyright holder saying it can be
distributed under the terms of this License.  Such a notice grants a
world-wide, royalty-free license, unlimited in duration, to use that
work under the conditions stated herein.  The ``Document'', below,
refers to any such manual or work.  Any member of the public is a
licensee, and is addressed as ``you''.  You accept the license if you
copy, modify or distribute the work in a way requiring permission
under copyright law.

A ``Modified Version'' of the Document means any work containing the
Document or a portion of it, either copied verbatim, or with
modifications and/or translated into another language.

A ``Secondary Section'' is a named appendix or a front-matter section of
the Document that deals exclusively with the relationship of the
publishers or authors of the Document to the Document's overall subject
(or to related matters) and contains nothing that could fall directly
within that overall subject.  (Thus, if the Document is in part a
textbook of mathematics, a Secondary Section may not explain any
mathematics.)  The relationship could be a matter of historical
connection with the subject or with related matters, or of legal,
commercial, philosophical, ethical or political position regarding
them.

The ``Invariant Sections'' are certain Secondary Sections whose titles
are designated, as being those of Invariant Sections, in the notice
that says that the Document is released under this License.  If a
section does not fit the above definition of Secondary then it is not
allowed to be designated as Invariant.  The Document may contain zero
Invariant Sections.  If the Document does not identify any Invariant
Sections then there are none.

The ``Cover Texts'' are certain short passages of text that are listed,
as Front-Cover Texts or Back-Cover Texts, in the notice that says that
the Document is released under this License.  A Front-Cover Text may
be at most 5 words, and a Back-Cover Text may be at most 25 words.

A ``Transparent'' copy of the Document means a machine-readable copy,
represented in a format whose specification is available to the
general public, that is suitable for revising the document
straightforwardly with generic text editors or (for images composed of
pixels) generic paint programs or (for drawings) some widely available
drawing editor, and that is suitable for input to text formatters or
for automatic translation to a variety of formats suitable for input
to text formatters.  A copy made in an otherwise Transparent file
format whose markup, or absence of markup, has been arranged to thwart
or discourage subsequent modification by readers is not Transparent.
An image format is not Transparent if used for any substantial amount
of text.  A copy that is not ``Transparent'' is called ``Opaque''.

Examples of suitable formats for Transparent copies include plain
ASCII without markup, Texinfo input format, \LaTeX\ input format, SGML
or XML using a publicly available DTD, and standard-conforming simple
HTML, PostScript or PDF designed for human modification.  Examples of
transparent image formats include PNG, XCF and JPG.  Opaque formats
include proprietary formats that can be read and edited only by
proprietary word processors, SGML or XML for which the DTD and/or
processing tools are not generally available, and the
machine-generated HTML, PostScript or PDF produced by some word
processors for output purposes only.

The ``Title Page'' means, for a printed book, the title page itself,
plus such following pages as are needed to hold, legibly, the material
this License requires to appear in the title page.  For works in
formats which do not have any title page as such, ``Title Page'' means
the text near the most prominent appearance of the work's title,
preceding the beginning of the body of the text.

A section ``Entitled XYZ'' means a named subunit of the Document whose
title either is precisely XYZ or contains XYZ in parentheses following
text that translates XYZ in another language.  (Here XYZ stands for a
specific section name mentioned below, such as ``Acknowledgements'',
``Dedications'', ``Endorsements'', or ``History''.)  To ``Preserve the Title''
of such a section when you modify the Document means that it remains a
section ``Entitled XYZ'' according to this definition.

The Document may include Warranty Disclaimers next to the notice which
states that this License applies to the Document.  These Warranty
Disclaimers are considered to be included by reference in this
License, but only as regards disclaiming warranties: any other
implication that these Warranty Disclaimers may have is void and has
no effect on the meaning of this License.


\section{VERBATIM COPYING}
\label{verbatim}

You may copy and distribute the Document in any medium, either
commercially or noncommercially, provided that this License, the
copyright notices, and the license notice saying this License applies
to the Document are reproduced in all copies, and that you add no other
conditions whatsoever to those of this License.  You may not use
technical measures to obstruct or control the reading or further
copying of the copies you make or distribute.  However, you may accept
compensation in exchange for copies.  If you distribute a large enough
number of copies you must also follow the conditions in
section~\ref{copying}.

You may also lend copies, under the same conditions stated above, and
you may publicly display copies.


\section{COPYING IN QUANTITY}
\label{copying}

If you publish printed copies (or copies in media that commonly have
printed covers) of the Document, numbering more than 100, and the
Document's license notice requires Cover Texts, you must enclose the
copies in covers that carry, clearly and legibly, all these Cover
Texts: Front-Cover Texts on the front cover, and Back-Cover Texts on
the back cover.  Both covers must also clearly and legibly identify
you as the publisher of these copies.  The front cover must present
the full title with all words of the title equally prominent and
visible.  You may add other material on the covers in addition.
Copying with changes limited to the covers, as long as they preserve
the title of the Document and satisfy these conditions, can be treated
as verbatim copying in other respects.

If the required texts for either cover are too voluminous to fit
legibly, you should put the first ones listed (as many as fit
reasonably) on the actual cover, and continue the rest onto adjacent
pages.

If you publish or distribute Opaque copies of the Document numbering
more than 100, you must either include a machine-readable Transparent
copy along with each Opaque copy, or state in or with each Opaque copy
a computer-network location from which the general network-using
public has access to download using public-standard network protocols
a complete Transparent copy of the Document, free of added material.
If you use the latter option, you must take reasonably prudent steps,
when you begin distribution of Opaque copies in quantity, to ensure
that this Transparent copy will remain thus accessible at the stated
location until at least one year after the last time you distribute an
Opaque copy (directly or through your agents or retailers) of that
edition to the public.

It is requested, but not required, that you contact the authors of the
Document well before redistributing any large number of copies, to give
them a chance to provide you with an updated version of the Document.


\section{MODIFICATIONS}
\label{modifications}

You may copy and distribute a Modified Version of the Document under
the conditions of sections~\ref{verbatim} and \ref{copying} above,
provided that you release
the Modified Version under precisely this License, with the Modified
Version filling the role of the Document, thus licensing distribution
and modification of the Modified Version to whoever possesses a copy
of it.  In addition, you must do these things in the Modified Version:

\renewcommand{\labelenumi}{\Alph{enumi}.}
\begin{enumerate}
\item Use in the Title Page (and on the covers, if any) a title distinct
   from that of the Document, and from those of previous versions
   (which should, if there were any, be listed in the History section
   of the Document).  You may use the same title as a previous version
   if the original publisher of that version gives permission.
\item List on the Title Page, as authors, one or more persons or entities
   responsible for authorship of the modifications in the Modified
   Version, together with at least five of the principal authors of the
   Document (all of its principal authors, if it has fewer than five),
   unless they release you from this requirement.
\item State on the Title page the name of the publisher of the
   Modified Version, as the publisher.
\item Preserve all the copyright notices of the Document.
\item Add an appropriate copyright notice for your modifications
   adjacent to the other copyright notices.
\item Include, immediately after the copyright notices, a license notice
   giving the public permission to use the Modified Version under the
   terms of this License, in the form shown in the Addendum below.
\item Preserve in that license notice the full lists of Invariant Sections
   and required Cover Texts given in the Document's license notice.
\item Include an unaltered copy of this License.
\item Preserve the section Entitled ``History'', Preserve its Title, and add
   to it an item stating at least the title, year, new authors, and
   publisher of the Modified Version as given on the Title Page.  If
   there is no section Entitled ``History'' in the Document, create one
   stating the title, year, authors, and publisher of the Document as
   given on its Title Page, then add an item describing the Modified
   Version as stated in the previous sentence.
\item Preserve the network location, if any, given in the Document for
   public access to a Transparent copy of the Document, and likewise
   the network locations given in the Document for previous versions
   it was based on.  These may be placed in the ``History'' section.
   You may omit a network location for a work that was published at
   least four years before the Document itself, or if the original
   publisher of the version it refers to gives permission.
\item For any section Entitled ``Acknowledgements'' or ``Dedications'',
   Preserve the Title of the section, and preserve in the section all
   the substance and tone of each of the contributor acknowledgements
   and/or dedications given therein.
\item Preserve all the Invariant Sections of the Document,
   unaltered in their text and in their titles.  Section numbers
   or the equivalent are not considered part of the section titles.
\item Delete any section Entitled ``Endorsements''.  Such a section
   may not be included in the Modified Version.
\item Do not retitle any existing section to be Entitled ``Endorsements''
   or to conflict in title with any Invariant Section.
\item Preserve any Warranty Disclaimers.

\end{enumerate}

If the Modified Version includes new front-matter sections or
appendices that qualify as Secondary Sections and contain no material
copied from the Document, you may at your option designate some or all
of these sections as invariant.  To do this, add their titles to the
list of Invariant Sections in the Modified Version's license notice.
These titles must be distinct from any other section titles.

You may add a section Entitled ``Endorsements'', provided it contains
nothing but endorsements of your Modified Version by various
parties--for example, statements of peer review or that the text has
been approved by an organization as the authoritative definition of a
standard.

You may add a passage of up to five words as a Front-Cover Text, and a
passage of up to 25 words as a Back-Cover Text, to the end of the list
of Cover Texts in the Modified Version.  Only one passage of
Front-Cover Text and one of Back-Cover Text may be added by (or
through arrangements made by) any one entity.  If the Document already
includes a cover text for the same cover, previously added by you or
by arrangement made by the same entity you are acting on behalf of,
you may not add another; but you may replace the old one, on explicit
permission from the previous publisher that added the old one.

The author(s) and publisher(s) of the Document do not by this License
give permission to use their names for publicity for or to assert or
imply endorsement of any Modified Version.


\section{COMBINING DOCUMENTS}
\label{combining}

You may combine the Document with other documents released under this
License, under the terms defined in section~\ref{modifications}
above for modified
versions, provided that you include in the combination all of the
Invariant Sections of all of the original documents, unmodified, and
list them all as Invariant Sections of your combined work in its
license notice, and that you preserve all their Warranty Disclaimers.

The combined work need only contain one copy of this License, and
multiple identical Invariant Sections may be replaced with a single
copy.  If there are multiple Invariant Sections with the same name but
different contents, make the title of each such section unique by
adding at the end of it, in parentheses, the name of the original
author or publisher of that section if known, or else a unique number.
Make the same adjustment to the section titles in the list of
Invariant Sections in the license notice of the combined work.

In the combination, you must combine any sections Entitled ``History''
in the various original documents, forming one section Entitled
``History''; likewise combine any sections Entitled ``Acknowledgements'',
and any sections Entitled ``Dedications''.  You must delete all sections
Entitled ``Endorsements''.


\section{COLLECTIONS OF DOCUMENTS}
\label{collections}

You may make a collection consisting of the Document and other documents
released under this License, and replace the individual copies of this
License in the various documents with a single copy that is included in
the collection, provided that you follow the rules of this License for
verbatim copying of each of the documents in all other respects.

You may extract a single document from such a collection, and distribute
it individually under this License, provided you insert a copy of this
License into the extracted document, and follow this License in all
other respects regarding verbatim copying of that document.


\section{AGGREGATION WITH INDEPENDENT WORKS}
\label{aggregation}

A compilation of the Document or its derivatives with other separate
and independent documents or works, in or on a volume of a storage or
distribution medium, is called an ``aggregate'' if the copyright
resulting from the compilation is not used to limit the legal rights
of the compilation's users beyond what the individual works permit.
When the Document is included in an aggregate, this License does not
apply to the other works in the aggregate which are not themselves
derivative works of the Document.

If the Cover Text requirement of section~\ref{copying} is applicable to
these copies of the Document, then if the Document is less than one half
of the entire aggregate, the Document's Cover Texts may be placed on
covers that bracket the Document within the aggregate, or the
electronic equivalent of covers if the Document is in electronic form.
Otherwise they must appear on printed covers that bracket the whole
aggregate.


\section{TRANSLATION}
\label{translation}

Translation is considered a kind of modification, so you may
distribute translations of the Document under the terms of
section~\ref{modifications}.
Replacing Invariant Sections with translations requires special
permission from their copyright holders, but you may include
translations of some or all Invariant Sections in addition to the
original versions of these Invariant Sections.  You may include a
translation of this License, and all the license notices in the
Document, and any Warranty Disclaimers, provided that you also include
the original English version of this License and the original versions
of those notices and disclaimers.  In case of a disagreement between
the translation and the original version of this License or a notice
or disclaimer, the original version will prevail.

If a section in the Document is Entitled ``Acknowledgements'',
``Dedications'', or ``History'', the requirement
(section~\ref{modifications}) to Preserve
its Title (section~\ref{applicability}) will typically require
changing the actual title.


\section{TERMINATION}
\label{termination}

You may not copy, modify, sublicense, or distribute the Document except
as expressly provided for under this License.  Any other attempt to
copy, modify, sublicense or distribute the Document is void, and will
automatically terminate your rights under this License.  However,
parties who have received copies, or rights, from you under this
License will not have their licenses terminated so long as such
parties remain in full compliance.


\section{FUTURE REVISIONS OF THIS LICENSE}
\label{future}

The Free Software Foundation may publish new, revised versions
of the GNU Free Documentation License from time to time.  Such new
versions will be similar in spirit to the present version, but may
differ in detail to address new problems or concerns.  See
http://www.gnu.org/copyleft/.

Each version of the License is given a distinguishing version number.
If the Document specifies that a particular numbered version of this
License ``or any later version'' applies to it, you have the option of
following the terms and conditions either of that specified version or
of any later version that has been published (not as a draft) by the
Free Software Foundation.  If the Document does not specify a version
number of this License, you may choose any version ever published (not
as a draft) by the Free Software Foundation.


\section*{ADDENDUM: How to use this License for your documents}

To use this License in a document you have written, include a copy of
the License in the document and put the following copyright and
license notices just after the title page:

\begin{quote}
    Copyright \copyright\ YEAR  YOUR NAME.
    Permission is granted to copy, distribute and/or modify this document
    under the terms of the GNU Free Documentation License, Version 1.2
    or any later version published by the Free Software Foundation;
    with no Invariant Sections, no Front-Cover Texts, and no Back-Cover Texts.
    A copy of the license is included in the section entitled ``GNU
    Free Documentation License''.
\end{quote}

If you have Invariant Sections, Front-Cover Texts and Back-Cover Texts,
replace the ``with...Texts.'' line with this:

    with the Invariant Sections being LIST THEIR TITLES, with the
    Front-Cover Texts being LIST, and with the Back-Cover Texts being LIST.

If you have Invariant Sections without Cover Texts, or some other
combination of the three, merge those two alternatives to suit the
situation.

If your document contains nontrivial examples of program code, we
recommend releasing these examples in parallel under your choice of
free software license, such as the GNU General Public License,
to permit their use in free software.


==> hyperref/hyperref.tex <==
\foilhead{Bookmarks with package *hyperref*}
\begin{itemize}
\item Places for options.
\item Options for bookmarks.
\item Creating bookmarks.
\item Replacement methods.
\end{itemize}

\begingroup
\hypersetup{bookmarksopenlevel=2}

\subfoilhead{Places for \texorpdfstring{*hyperref* }{}options}
\begin{enumerate}
\item Global: \Blue{\cms{documentclass}}\Code{[}\dots\Code{]} (*eg* driver)
\item Package: \Blue{\cms{usepackage}}\Code{[}\dots\Code{]}
\item Configuration file: \Blue{\File{hyperref.cfg}} with \cms{hypersetup}
\item After package has been loaded:
  \Blue{\cms{hypersetup}}\Code{\{}\dots\Code{\}}\\
  (*eg* *pdf* information options)
\end{enumerate}


\subfoilhead[-1.5\baselineskip]{Bookmark options}

\begingroup
  \def\sep{0.5ex}
  \noindent
  \Red{\Option{bookmarks}}: Make bookmarks
    (default: \Green{\Value{true}}).\\[\sep]
  \Red{\Option{bookmarksnumbered}}: Put section numbers in bookmarks
    (\Green{\Value{false}}).\\[\sep]
  \Red{\Option{bookmarksopen}}: Open up bookmark tree
     (default: \Green{\Value{false}}).\\[\sep]
  \Red{\Option{bookmarksopenlevel}}: Level, to which bookmarks are
     open.\\[\sep]
  \Red{\Option{pdfpagemode}}: How document starts when opened
     (default: \Green{\Value{None}}):
  \begingroup
    \mbox\qquad\Blue{\Option{None}}: Neither outlines nor thumbnails are visible.\\
    \mbox\qquad\Blue{\Option{UseOutlines}}, \Blue{\Option{UseThumbs}}:
      Outlines, thumbnails are visible.\\
    \mbox\qquad\Blue{\Option{FullScreen}}: Full-screen mode.\\[\sep]
  \endgroup
  \Red{\Option{unicode}}: Bookmarks in *unicode*
     (\Green{\Value{false}}). After package has been\\
     \mbox\qquad loaded, it switches between *unicode* and *pdfdocencoding*.
\endgroup


\subfoilhead[-0.5\baselineskip]{%
  \texorpdfstring{Bookmarks by \abbr{sectioning}}{\abbr{Sectioning}} %
  commands
}
\label{sec:bmbysec}

\begin{itemize}
\item Automatically addition of bookmarks by:
      \begin{itemize}
      \item \cms{part}, \cms{chapter}, \cms{section}, \cms{subsection}, \dots
      \item \cms{addcontentsline}
      \end{itemize}
\item Help file \Blue{\Code{\textsl{\cms{jobname}}.out}}:
      \begin{itemize}
      \item It is written in the \Green{first} run.
      \item The bookmarks are set in the \Green{second} run.
      \item There is \Green{\emph{no}} ``rerun'' warning.
      \end{itemize}
\end{itemize}


\subfoilhead{Tree structure\texorpdfstring{ of bookmarks}{}}

\begin{itemize}
\item Subentries must be added to \Blue{direct} ancestores,
      \Blue{not} grandparents.
\item If an intermediate level is omitted, the leaf starts \Blue{leftmost}:
      \begin{quote}
        \def\sub{\Red{\ensuremath{\rightarrow}}}%
        \def\ver{\Red{\ensuremath{\|}}}%
        \begin{tabular}{@{}lll@{}}
        &\Blue{table of contents}&\Blue{bookmarks}\\
        \hline
        \cms{part}\Code{\{I\}}&\ver{Part I}&\ver{main entry}\\
        \cms{chapter}\Code{\{5\}}&%
          \ver\sub{Chapter I.5}&\ver\sub{subentry}\\
        \cms{subsection}\Code{\{1\}}&
          \ver\sub\sub\sub{Subsection I.5.0.1}&\ver{main entry}\\
        \end{tabular}
      \end{quote}
\end{itemize}


\subfoilhead[-\baselineskip]{\texorpdfstring{Creating bookmarks with }{}\cms{pdfbookmark}}

\begin{itemize}
\item The bookmarks of *sectioning* commands have an \Red{level} number:
      \par\noindent
      \begin{tabular}{@{}lc@{ }c@{ }c@{ }c@{ }c@{}}
      documentclass&\cms{part}&\cms{chapter}&%
        \cms{section}&\cms{subsection}&\dots\\
      \Class{book}/\Class{report}:&\Red{\llap{$-$}1}&%
        \Red0&\Red1&\Red2&\dots\\
      \Class{article}:&\Red0&&\Red1&\Red2&\dots\\
      \end{tabular}
\item Syntax of \Blue{\cms{pdfbookmark}} (default for level: \Red{0}):
      \begin{quote}
        \Blue{\cms{pdfbookmark}}%
          \Code{[\Red{\emph{level}}]\{\emph{bookmark text}\}%
            \{\Green{\emph{anchor name}}\}}
      \end{quote}
\item \Blue{\cms{currentpdfbookmark}}%
        \Code{\{\emph{bookmark}\}\{\Green{\emph{anchor}}\}}%
        \commentchar\ \Red{current level}
\item \Blue{\cms{subpdfbookmark}}%
        \Code{\{\emph{bookmark}\}\{\Green{\emph{anchor}}\}}%
        \commentchar\ \Red{current level + 1}
\end{itemize}


\subsubfoilhead[-\baselineskip]{Using anchors%
  \texorpdfstring{ with \cms{pdfbookmark}}{}%
}

\begin{itemize}
\item An \Green{anchor name} consists of the argument and
      the level:
      \begin{quote}
        \Blue{\cms{pdfbookmark}}\Code{[\Red0]\{Titlepage\}\{\Green{tit}\}}%
          \Code{\commentchar\ }anchor: \Code{\Green{tit}.\Red0}
      \end{quote}
\item The bookmark can point to another \Green{target} (\Green{anchor}):
      \begin{quote}\small
        \cms{hypertarget}\Code{\{\Green{place.}\Red{1}\}\{\}}
      \end{quote}
      Redirecting the bookmark to the previous defined \Green{target}:
      \begin{quote}\small
        \cms{begingroup}\\
        *ind*\cms{makeatletter}\\
        *ind*\cms{def}\cms{hyper@anchorstart}\Code{ \#1}%
          \cms{hyper@anchorend}\Code{\{\}\%}\\
        *ind*\Blue{\cms{pdfbookmark}}\Code{[\Red1]\{Go to the place\}\{\Green{place}\}\%}\\
        \cms{endgroup}
      \end{quote}
\end{itemize}

\endgroup
\endinput


==> hyperref/links.tex <==
\subfoilhead[-\baselineskip]{Links}

\begin{Nav}{\NavBookmarks\NavQuit}

\begin{smallpar}
\let\Blue\empty
\pdfadjustspacing=1
\noindent
\begingroup
\def\it{\textbullet}%
\def\sep{1ex}%
\begin{tabularx}{\linewidth}{@{}l@{ }X@{}}
  \it&\Blue{*pdfspec*} (version 1.3):\newline
    \link{http://partners.adobe.com/asn/developer/PDFS/TN/PDFSPEC.PDF}%
    \tabularnewline[\sep]
  \it&\Blue{*pdftex*}:
    \begingroup
      \settoheight{\dimen0}{\mbox{\^e}}%
      \settoheight{\dimen1}{\mbox{e}}%
      \addtolength{\dimen0}{-\dimen1}%
    (H\`an Th\rlap{\raise\dimen0\hbox{\'{}}}\^e Th\`anh):
    \endgroup
    \newline
    \link{http://www.tug.org/applications/pdftex/}\newline
    Win32: \link{ftp://ftp.ese-metz.fr/pub/TeX/win32-beta/}%
    \tabularnewline[\sep]
  \it&\Blue{*hyperref*} (Sebastian Rahtz):\hfill
    \link{ftp://ctan.tug.org/tex-archive/macros/latex/contrib/supported/hyperref/}%
    \newline
    Test versions:\newline
    \link{http://www.tug.org/applications/hyperref/hyperref.zip}
    \tabularnewline[\sep]
  \it&\Blue{*hypbmsec*} (Heiko Oberdiek):\hfill
    \link{ftp://ctan.tug.org/tex-archive/macros/latex/contrib/supported/oberdiek/}%
    \tabularnewline[\sep]
  \it&\Blue{*thumbpdf*} (Heiko Oberdiek):\newline
    \link{ftp://ctan.tug.org/tex-archive/macros/pdftex/thumbpdf/}%
\end{tabularx}
\endgroup
\end{smallpar}

%\SetNav{\NavFull\NavSep\NavPrev\NavSep\NavQuit}
\end{Nav}

\endinput


==> hyperref/navbook.tex <==
\newcommand{\bmaction}[3][0]{%
  \begingroup
    \pdfstringdef\x{#3}%
    \pdfoutline user {<</S /Named /N /#2>>} count #1 {\x}%
  \endgroup
}
\bmaction[-3]{NOP}{Navigation}
  \bmaction[2]{FullScreen}{Full-screen}
    \bmaction{PageOnly}{Page only}
    \bmaction{ShowThumbs}{Thumbnails}
  \bmaction[6]{NOP}{Selecting pages}
    \bmaction{PrevPage}{Previous page}
    \bmaction{NextPage}{Next page}
    \bmaction{GoBack}{Go back}
    \bmaction{GoForward}{Go forward}
    \bmaction{FirstPage}{First page}
    \bmaction{LastPage}{Last page}
  \bmaction[2]{GeneralInfo}{General document information}
    \bmaction{ShowHideMenuBar}{Menu bar}
    \bmaction{ShowHideToolBar}{Tool bar}

\endinput


==> hyperref/pdfextra.tex <==
\foilhead{Additional features of \abbr{pdf} format}
\noindent
Hyperref does not support all possibilities of *pdf* format, e.\,g.:
\begin{itemize}
  \let\Blue\empty
  \item \Blue{\Code{/CreationDate}} and \Blue{\Code{/ModDate}}.
  \item \Blue{Bookmarks} with \Blue{other functions}.
\end{itemize}
The following examples uses commands of \empty{*pdftex*}.

\subfoilhead{Bookmarks with other functions}
\begin{Nav}{\NavBookmarks\NavPage}

\begin{itemize}
  \item Menu functions of AcrobatReader, sound, video, \dots
  \item *pdftex* low level command:\\[1ex]
        \code[red]<\pdfoutline>\ \emph{\code<action>}\
        \code<count>\ \emph{\code[blue]<n>}\
        \code<{>\emph{\code<text>}\code<}>
        \begin{itemize}
          \item
            The absolute value of \emph{\code[blue]<n>}\ is the
            count of the direct subentries.
          \item
            If \emph{\code[blue]<n>}\ is negative, the
            subentries are closed.
        \end{itemize}
\end{itemize}


\subfoilhead{Link to external file}
\noindent
The *pdfspec* contains the possible actions on page 96.\\
At last a bookmark that points to that page:
\begingroup
  \edef\({\string(}
  \edef\){\string)}
\begin{verbatim}
$Blue(\pdfoutline)
  user {<<$Green(/S /GoToR /F $(pdfspec.pdf$) /D [95 /Fit])>>}
  count 0 {$empty(Description of actions)}
\end{verbatim}
\endgroup

\end{Nav}

\endinput


==> hyperref/pdfinfo.tex <==
\hypersetup!{%
  pdftitle!    = {PDF information and navigation elements},
  pdfsubject!  = {Slides for talk at EuroTeX'99 in Heidelberg},
  pdfkeywords! = {pdf, hyperref, bookmarks, thumbnails},
  pdfauthor!   = {\textcopyright\ Heiko Oberdiek},
  pdfcreator!  = {\LaTeX\ with package \flqq hyperref\frqq},
  pdfproducer! = {pdfeTeX-0.\the\pdftexversion\pdftexrevision},
}
\pdfinfo!{/CreationDate! (D:19990909000000-01'00')}

==> hyperref/psd.tex <==

\foilhead[-\baselineskip]{\cms{pdfstringdef}%
  \texorpdfstring{  converts \abbr{tex} to \abbr{pdf} strings}{}}

\noindent
Syntax: \Blue{\cms{pdfstringdef}}\Code{\{\emph{\cms{command}}\}%
    \{\emph{*tex* string}\}}

\begin{enumerate}
\item Selecting the encoding *PD1* or *PU*.
\item Redefinitions of many commands, so that they
      produce correct\\
      results or do not harm.
\item Expansion of the string.
\item Token checks and removal of forbidden tokens with 
      comprehensive\\ 
      warnings.
\end{enumerate}


\subfoilhead[-.5\baselineskip]{Redefinitions%
  \texorpdfstring{ by \cms{pdfstringdef}}{}}
\begin{itemize}
\item Redefinitions to get correct results, *eg*:
      \begin{itemize} 
      \item Glyph commands: \cms{\{}, \cms{\%}, \cms{space}, \cms{dots},
            \dots
      \item Logos: \cms{TeX}, \cms{LaTeX}, \cms{MF}, \dots
      \end{itemize}
\item Many tokens are removed silently, *eg*:
      \begin{itemize}
      \item *latex* commands: \cms{label}, \cms{index}, 
           \cms{textbf}, \dots
      \item Stomach tokens: curly group braces, \cms{relax} (\cms{protect}), 
            \dots
      \end{itemize}
\item The behaviour of \cms{xspace} is simulated.
\end{itemize}

\endinput


==> hyperref/replace.tex <==
\foilhead{Replacement methods}

\begin{itemize}
%\item \code[blue]<\texorpdfstring>\ provides an alternative.
\item \Blue{\cms{texorpdfstring}} choices one of its arguments:\\
      a *tex* or a *pdf* string.
\item \code[blue]<\pdfstringdefPreHook>\ is a place for redefining commands.\\
      Additions are made by \code[blue]<\pdfstringdefDisableCommands>.
\item Package \Blue{*hypbmsec*} extends the \code<\section>\ commands.
\end{itemize}


\subfoilhead{\cms{texorpdfstring} method}
\noindent
Syntax: \Red{\cms{texorpdfstring}}%
        \Green{\Code{\{*tex* string\}}}%
        \Blue{\Code{\{*pdf* string\}}}

\noindent
Example:

\noindent
  \cms{section}\Code{\{}\Red{\cms{texorpdfstring}}%
  %\Code{\emph{\%}}%
  \Green{\Code{\{H\$\_2\$O\}}}%
  %\Code{\emph{\%}}%
  \Blue{\Code{\{Water\}}}%
  %\Code{\emph{\%}}%
  \Code{\}}


\subfoilhead[-1\baselineskip]{Hook for private macro redefinitions}

\begin{itemize}
\item \Red{\cms{pdfstringdefPreHook}} is called, before expanding the string.
\item \Red{\cms{pdfstringdefDisableCommands}} adds user redefinitions to\\
      \cms{pdfstringdefPreHook}

  \Blue{\cms{pdfstringdefDisableCommands}}\Code{\{\commentchar}\\
  *ind*\cms{renewcommand}\Code{\{\cms{textcolor}\}[1]\{\#1\}\commentchar}\\
  *ind*\cms{renewcommand}\Code{\{\cms{url}\}}\Code{\{}\empty{\cms{pdfstringdefwarn}}%
    \Code{\{\cms{url}\}}\Code{\}\commentchar}\\
  *ind*\cms{let}\cms{textcolor}\cms{@gobble}\\
  \Code{\}}
\item \Red{\cms{pdfstringdefwarn}} prints a warning message.
\end{itemize}


\subfoilhead[-\baselineskip]{Package \Package{hypbmsec}}

\begin{itemize}
\item The syntax of \cms{section} commands is extended:
      \begin{itemize}
      \item Second optional bookmark argument.
      \item Bookmark in parentheses.
      \end{itemize}
\item Syntax:
  \def\txt{\Blue{\textsl{text}}}%
  \def\toc{\Green{\textsl{toc/head}}}%
  \def\out{\Red{\textsl{bookmark}}}%
  \settowidth{\dimen0}{\toc}%
  \settowidth{\dimen1}{\out}%
  \addtolength{\dimen1}{-\dimen0}%
  \setlength{\dimen1}{.5\dimen1}%
  \edef\toc{\noexpand\Green{\noexpand\textsl{toc%
    \noexpand\hspace{\the\dimen1}/\noexpand\hspace{\the\dimen1}head}}}%
  \settowidth{\dimen0}{\textbf{]\{}}%
  \settowidth{\dimen1}{ = }%
  \addtolength{\dimen0}{-\dimen1}%
  \setlength{\dimen0}{-.5\dimen0}%
  \edef\xsp{\noexpand\hspace{\the\dimen0}}%
  \def\({\textbf{(}\,}%
  \def\){\,\textbf{)}}%
  \def\[{\textbf{[}\,}%
  \def\]{\,\textbf{]}}%
  \def\{{\textbf{\orgbraceleft}\,}%
  \def\}{\,\textbf{\orgbraceright}}%
  \def\section{\cms{section}}%
  \def~{ = }%
  \begin{tabular}[t]{@{}l@{ }c@{}c@{}c@{}c@{}c@{}l@{}}
    \section&\{&\toc&~&\out&~&\txt\}\\
    \section&\[&\toc&~&\out&\]\,\{&\txt\}\\[1ex]
    \section&\[&\toc&\]\,\[&\out&\]\,\{&\txt\}\\[1ex]
    \section&\(&\out&\)\,\{&\toc&~&\txt\}\\
    \section&\[&\toc&\]\,\(&\out&\)\,\{&\txt\}\\
    \section&\(&\out&\)\,\[&\toc&\]\,\{&\txt\}\\
  \end{tabular}
\end{itemize}


\endinput

The next version of package *hypbmsec* will know the
option \Blue{\Option{startotoc}}:
The starred *sectioning* commands are included in the table
of contents and in the outline tree automatically.
For options \Blue{\Option{infix}} and \Blue{\Option{prefix}}
see \secref{sec:addcontentsline}.

\endinput


==> hyperref/strings.tex <==
\clearpage
\pdfbookmark[0]{Strings}{string}

\begingroup
\hypersetup{bookmarksopenlevel=2}

\subfoilhead[-\baselineskip]{\abbr{pdf} strings}

\begin{itemize}
\item Examples, where *pdf* strings are used:
      \begin{quote}
      Bookmark names, information dictionaries, text annotations
      \end{quote}
\item *pdf* strings follow the *postscript* rules:
      \begin{itemize}
      \item Delimited by parentheses: \Code{\Blue{(}This is a string\Blue{)}}
      \item Escape sequences for white space, \Blue{\cms{(}}, \Blue{\cms{)}},
            \Blue{\cms{}\cms{}};\\
            octal notation, *eg*: `\"a\"o\"u\ss' = 
            \Code{(}\Blue{\cms{344}\cms{366}\cms{374}\cms{337}}\Code{)}
      \end{itemize}
\item 
%      $\vcenter{\mbox{%
        \begin{tabular}[t]{@{}l@{ }l@{}}
          \Blue{*pdfdocencoding*}:&8bit, superset of *isolatin1*\\
          \Blue{*unicode*}:&16bit, *acroread* version $\ge$ 4\\
        \end{tabular}%
%      }}$ 
\end{itemize}


\clearpage
\pdfbookmark[1]{\abbr{tex} strings}{strings}

\subsubfoilhead[-.5\baselineskip]{Digestion of \abbr{tex}}

\begingroup
\newenvironment{organ}[2]{%
  \begin{minipage}[t]{\linewidth}%
    \vspace{#2}%
    \begin{tabbing}%
      \begin{tabular}{@{\textbullet\ }l@{}}
        \multicolumn{1}{@{}l@{}}{%
%          \phantom{\textbullet\ }%
          \textbf{\large\Blue{#1}}}\\[0.5ex]
}{
      \end{tabular}%
    \end{tabbing}%
  \end{minipage}%
}

\makeatletter
\let\fbox\@firstofone

\noindent
\fbox{%
\begin{organ}{Eyes}{0pt}
  Reading input lines\\
  Catcodes are set
\end{organ}}%
\hfill
\fbox{%
\begin{organ}{Mouth}{2\baselineskip}
  Forming tokens\\
  Expansion of macros
\end{organ}}%
\hfill
\fbox{%
\begin{organ}{Stomach}{4\baselineskip}
  Assignments\\
  Typesetting
\end{organ}}%

\endgroup


\subsubfoilhead[-.5\baselineskip]{Differences between mouth and stomach}

\noindent
\begin{tabular}{@{}lll@{}}
  &\Blue{\textbf{mouth}}&
   \Blue{\textbf{stomach}}\\[1ex]
``zero'':& \code<\empty>&\code<\relax>\\[0.5ex]
\code<{...}>:&parameter&group\\[0.5ex]
variable:&read and check&assignments\\[0.5ex]
fonts:&--&different fonts and encodings\\
&&ligatures\\[0.5ex]
Commands:&\code<\string>, \code<\number>&\code<\def>, \code<\hbox>, \code<$>\\
&\code<\if>, \code<\the>&\code<\begingroup>, \code<\special>
\end{tabular}


\subfoilhead[-.5\baselineskip]{\abbr{tex} into \abbr{pdf} strings}

\begin{itemize}
\item Reusing the argument of *sectioning* commands (*tex* string)\\
      for the bookmarks (*pdf* strings).
\item Limitations because of missing stomach digestion:
      \begin{itemize}
      \item No manipulation of boxes, no mathematics, no colors, \dots
      \item No change of fonts or encodings, no ligatures.
      \item No assignments (\cms{xspace} uses \cms{futurelet}).
      \item Unexpandable commands appear verbatim.
      \end{itemize}
\end{itemize}


\endgroup
\endinput

==> hyperref/summary.tex <==
\clearpage
\pdfbookmark[0]{End}{ende}

\subfoilhead[-1.5\baselineskip]{Summary}
\begin{itemize}
  \item \Red{General document information}:
    \begin{itemize}
      \item Options in \code[blue]<\hypersetup>\
            after \cms{usepackage}\Code{\{hyperref\}}.
    \end{itemize}
  \item \Red{Bookmarks}:
    \begin{itemize}
      \item Automatically added by \Blue{*hyperref*}.
      \item \Blue{Oral expansion}, no stomach commands (exceptions).
      \item Replacement methods: \code[blue]<\texorpdfstring>,\\
            \code[blue]<\pdfstringdefDisableCommands>, and
            \Blue{*hypbmsec*}.
      \item Low level commands only for special effects.
    \end{itemize}
  \item \Red{Thumbnails}: Automatically added by \Blue{*thumbpdf*}.
\end{itemize}


==> hyperref/thumb.tex <==

\foilhead{Thumbnails}
\begin{Nav}{\NavThumbnails\NavBookmarks}
\thisthumb{zurueck}
\begin{itemize}
  \item Another method for navigation:
    \begin{itemize}
      \item Choosing pages.
      \item Selecting page areas.
    \end{itemize}
  \item Contents:
    \begin{itemize}
      \item Thumbnail sketches of the pages.
      \item Other pictograms, symbols, \dots
      \item Empty.
    \end{itemize}
\end{itemize}


\subfoilhead{Adding thumbnails with \abbr{thumbpdf}}
\thisthumb{weiter}
\begingroup
  \centering
  \setlength{\unitlength}{1pt}
  % ca. max: 240mm x 100mm
  % ca. max: 700pt x 300pt
  \def\FileBox#1{\framebox(180,40){\Code{\vphantom{Hg}#1}}}
  \def\ProgBox[#1]#2{\makebox(160,60)[#1]{\vphantom{Hg}#2}}
  \def\Nummer[#1]#2{\makebox(20,60)[#1]{%
    \vphantom{Hg}%
    $\smash{%
      \textsf{\textcircled{\vphantom{\large#2}\Blue{\small#2}}}%
    }$%
  }}
  \def\Down{\makebox(0,0)[b]{\DOWNarrow}}%
  \def\Up{\makebox(0,0)[t]{\UParrow}}%
  \def\Right{\makebox(0,0)[r]{\RIGHTarrow}}%
  \begin{picture}(670,250)
    % Dateinamen
    \put(80,0){\FileBox{thumbdta.tex}}
    \put(80,100){\FileBox{\emph{jobname}.pdf}}
    \put(80,200){\FileBox{\emph{jobname}.tex}}
    \put(470,200){\FileBox{\Red{\emph{jobname}.pdf}}}
    % Pfeile
    \put(170,200){\line(0,-1){60}}
    \put(170,140){\Down}
    \put(170,100){\line(0,-1){60}}
    \put(170,40){\Down}
    \put(260,220){\line(1,0){210}}
    \put(470,220){\Right}
    \put(260,20){\line(1,0){105}}
    \put(365,20){\line(0,1){160}}
    \put(365,180){\Up}
    % Nummern
    \put(190,140){\Nummer[l]{1}}
    \put(190,40){\Nummer[l]{2}}
    \put(280,230){\Nummer[lb]{3}}
    % Programme
    \put(-10,40){\ProgBox[r]{*thumbpdf*}}
    \put(-10,140){\ProgBox[r]{*pdftex*}}
    \put(285,230){\ProgBox[b]{*pdftex*}}
    \put(285,150){\ProgBox[t]{\Code{thumbpdf.sty}}}
  \end{picture}
\endgroup

\subfoilhead[-\baselineskip]{How \abbr{thumbpdf} works}
\begingroup
  \centering
  \setlength{\unitlength}{1pt}
  % ca. max: 240mm x 100mm
  % ca. max: 700pt x 300pt
  \def\FileBox#1{\framebox(180,40){\Code{\vphantom{Hg}#1}}}
  \def\ProgBox[#1]#2{\makebox(160,60)[#1]{\vphantom{Hg}#2}}
  \def\Down{\makebox(0,0)[b]{\DOWNarrow}}%
  \def\Up{\makebox(0,0)[t]{\UParrow}}%
  \def\Right{\makebox(0,0)[r]{\RIGHTarrow}}%
  \def\Left{\makebox(0,0)[l]{\LEFTarrow}}%
  \begin{picture}(650,340)
    % Dateinamen
    \put(80,0){\FileBox{\Red{thumbdta.tex}}}
    \put(80,100){\FileBox{thumbdta.pdf}}
    \put(80,200){\FileBox{thumb\emph{???}.png}}
    \put(80,300){\FileBox{\emph{jobname}.pdf}}
    \put(420,150){\FileBox{thumbopt.tex}}
    \put(420,240){\FileBox{\emph{other images}}}
    % Pfeile
    \put(170,300){\line(0,-1){60}}
    \put(170,240){\Down}
    \put(170,200){\line(0,-1){60}}
    \put(170,140){\Down}
    \put(170,100){\line(0,-1){60}}
    \put(170,40){\Down}
    \put(360,170){\line(1,0){60}}
    \put(360,170){\Left}
    \put(510,240){\line(0,-1){50}}
    \put(510,190){\Down}
    % Programme
    \put(-10,40){\ProgBox[r]{\textsf{perl}}}
    \put(-10,140){\ProgBox[r]{*pdftex*}}
    \put(190,140){\ProgBox[l]{\Code{thumbpdf.tex}}}
    \put(-10,240){\ProgBox[r]{*gs*}}
  \end{picture}
\endgroup


\iffalse %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subfoilhead{Thumbnails and *pdftex*}
\begin{itemize}
\item There is no direct support.
\item \code[blue]<\pdfimage> (*pdftex* versions below 0.14):
  \begin{itemize}
    \item[$+$] Image works as thumbnail.
    \item[$-$] No access to the image object number.
    \item[$-$] Image is on the page, must be
               moved out of the page.
  \end{itemize}
\item Low level commands
  \code[blue]<\pdfobj>\ and \code[blue]<\pdflastobj>\ are possible.
\end{itemize}

\clearpage
\pdfbookmark[1]{Project *thumbpdf*}{thumbpdf}
\subsubfoilhead[-\baselineskip]{Solution\texorpdfstring{ of project *thumbpdf*}{}}

\begin{enumerate}
  \item Generating the thumbnails \Blue{\file{thumb???.png}} by \Red{*gs*}.
  \item \Red{*pdftex*} runs \Red{\file{thumbpdf.tex}},
        thumbnails included by \code[blue]<\pdfimage>.
  \item The perl script \Red{\file{thumbpdf.pl}} reads
        \Blue{\file{thumbpdf.pdf}} and writes\\
        the object data in a *tex*
        readable form \Blue{\file{thumbdta.tex}}.
  \item Package \Red{\file{thumbpdf.sty}} inputs \Blue{\file{thumbdta.tex}},
        that contains the\\
        thumbnails as *pdf* objects (\code[blue]<\pdfobj>).
  \item The object numbers of the thumbnails (\code[blue]<\pdflastobj>)
        are added\\
        to the page attributes (\code[blue]<\pdfpageattr>).
\end{enumerate}


\subsubfoilhead[-.5\baselineskip]{User interface\texorpdfstring{ of *thumbpdf*}{}}

\begin{itemize}
  \def\master{\textsl{master}}%
  \item Command lines (\file{\master.tex} inputs \file{thumbpdf.sty}):
    \begin{enumerate}
      \item \texttt{\Blue{pdf}(\Blue{e},\Blue{la})\Blue{tex \master.tex}}
      \item \Blue{\texttt{thumbpdf \master}}
      \item \texttt{\Blue{pdf}(\Blue{e},\Blue{la})\Blue{tex \master.tex}}
    \end{enumerate}
  \item Another program than *gs* can be used:
    \begin{enumerate}
      \item[2a.] \Blue{\texttt{\textsl{ProgramThatGeneratesThumbnails} \master.pdf}}
      \item[2b.] \Blue{\texttt{thumbpdf}}
    \end{enumerate}
\end{itemize}

\fi %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subfoilhead[-\baselineskip]{Other images as thumbnails}

\begin{itemize}
\item With \Blue{\cms{thumb}} other images are declared as
      thumbnails in the\\ 
      optional file \Blue{\file{thumbopt.tex}}.
\item \Blue{\cms{thisthumb}} sets the thumbnail for the current page.
\end{itemize}
\begingroup
  \let\Red\Green
  \centering
  \begin{tabular}{@{}l@{\quad$\rightarrow$\quad}l@{}}
    \multicolumn{1}{@{}l}{\empty{\File{thumbopt.tex}}}&%
      \File{\emph{jobname}.tex}\\
    \hline
    \empty{\cms{thumb}}\Code{\{\Red{one}\}}&
      \empty{\cms{thisthumb}}\Code{\{\Red{one}\}}\\
    \empty{\cms{thumb}}\Code{\{\Red{one.png}\}}&
      \empty{\cms{thisthumb}}\Code{\{\Red{one.png}\}}\\
    \empty{\cms{thumb}}\Code{[\Red{two}]\{one\}}&
      \empty{\cms{thisthumb}}\Code{\{\Red{two}\}}\\
    \empty{\cms{thumb}}\Code{[\Red{one}]\{./extras/one.png\}}&
      \empty{\cms{thisthumb}}\Code{\{\Red{one}\}}\\
  \end{tabular}
  \par
\endgroup

\end{Nav}

\endinput


==> hyperref/thumbopt.tex <==
\thumb[zurueck]{addthumb/thumb001.png}
\thumb[weiter]{addthumb/thumb002.png}


==> hyperref/title.tex <==
\pdfbookmark[0]{Beginning}{anfang}
\pdfbookmark[1]{Title}{title}

%\date{21st September 1999}% EuroTeX'99
\date{13rd October 1999}% first release for hyperref
\title{*pdf* information and navigation elements with
       hyperref, *pdftex*, and thumbpdf}
\author{Heiko Oberdiek\\\Email{oberdiek@ruf.uni-freiburg.de}}

\begingroup
  \LogoOff\aftergroup\LogoOn
  \Restriction{\unskip\centerline{\NavStart}}%
  \aftergroup\Restriction\aftergroup\empty
  \maketitle
  \begin{abstract}
    \noindent
    Additional possibilities for information and navigation through
    paper-less on-line documents that offer the PDF format.
  \end{abstract}
  \newpage
\endgroup

\subfoilhead{Subjects}
\begin{itemize}
\item General document information\hfill*hyperref*
\item Bookmarks/outlines\hfill*hyperref*
\item Thumbnails\hfill*thumbpdf*
\end{itemize}

\endinput


==> ly1/README <==
LaTeX support for `texnansi' encoding (LY1)
===========================================

Installing
==========

Ordinarily, you don't have to do anything, since this package is likely
already present in your TeX distribution (TeX Live, MiKTeX).

But if you're on your own, then just recursively copy the directories
here to your texmf-local (or some) tree, preserving structure.  Then add
the map files *8y.map to your dvips setup and/or update the
configuration of other DVI drivers correspondingly.  You will have to
adjust URW vs. Adobe names as needed.  (In TeX Live, this is already
done in dvips35.map, etc., in conjunction with updmap, and the *8y.map
files here are not used.)

Usage
=====

The font encoding `LY1' corresponds to the `texnansi' encoding as used
by default in the Y&Y TeX system (http://tug.org/yandy).  There is also
an option to support the `ansinew' encoding that is the default encoding
in Microsoft Windows.

The main file is ly1enc.def. This contains the declaration of
the encoding. To use `texnansi' encoded fonts within LaTeX, 
typically you just need to add the line

	\usepackage[LY1]{fontenc}

to your document preamble.

An alternative to the above line is to use the `texnansi' package

	\usepackage{texnansi}

This will call the fontenc package, as above, to set up the LY1
encoding but then make further changes to the uppercase and
lowercase tables.  Note that LaTeX does not need these changes to
correctly uppercase text as its \MakeUppercase and \MakeLowercase
commands only require the uppercase and lower case codes of the
letters a-z.

So for most purposes it is better to use the call to fontenc
rather than use the `texnansi' package.  Then, if you pass the
file to a site using T1 (Cork) encoded fonts the line can more
easily be changed to

	\usepackage[T1]{fontenc}

The texnansi package has a package option `ansinew' which
modifies the LY1 encoding to refer to that MS Windows
encoding.  However you should only do this if your TeX system
can not reencode fonts to support T1 or LY1.  The `ansinew'
treatment of the left quote ` as a grave accent makes it
rather unsuitable for TeX use.  It also lacks several useful
glyphs.  However if you need to, you can do:

	\usepackage[ansinew]{texnansi}

The other possible reason for using the `texnansi' package
relates to the use of the lowercase table in the hyphenation
algorithm.  This is described below, but it is unfortunately
of necessity rather technical, and you may want to stop
reading at that point.

LY1 matches OT1 well enough that you can usually use it in that role
also.  You can \input texnansi if you want this to work exactly even in
plain TeX.

Having declared the LY1 encoding to LaTeX, LaTeX will need to
know the fonts that are available in this encoding.  This
distribution includes TeX metrics, font definition files and
map files for the common `Standard PostScript' fonts.

For each encoding LaTeX needs to know an `error font' which is
its fall back in the case that the font substitution system
can find nothing better to do.  ly1enc.def specifies that the
Error Font for LY1 is Adobe Times-Roman.  Any PostScript
interpreter must be able to provide Times-Roman, so it seems a
good choice as the error font.  Yet you may wish to change
this for any reason; just edit the lines

\DeclareErrorFont{LY1}{ptm}{m}{n}{10}
\DeclareFontSubstitution{LY1}{ptm}{m}{n}

at the top of ly1enc.def to refer to some other font set.  For example
if you have Y&Y TeX's `Lucida Bright' distribution you could change the
two occurrences of {ptm} to {hlh} to make LaTeX fall back on Lucida
Bright if all else fails.  Please follow the LPPL and do not
capriciously alter ly1enc.def in other ways.

For more information on LY1 encoding and see Y&Y's WWW page:

        <http://www.tug.org/yandy/usely1.htm>
        

A Note on Lowercase Codes and Hyphenation Tables
================================================

The lowercase table is used by TeX's hyphenation algorithm, so
in principle one would need to change the lowercase table to
match the encoding used.  However, it should not be changed
mid paragraph as all words, whatever font encoding they are
set in, are lowercased using the table current at the *end* of
the paragraph before being checked for hyphenation.  Because
of these limitations in TeX's hyphenation algorithm, LaTeX
does not support changing the lowercase table mid document, so
if the `texnansi' package is used then the `texnansi'
lowercase table will be used for all fonts (whether or not LY1
encoded) and conversely if it is not used, the T1 table will
be used, even for LY1 encoded fonts.  The reason why this
problem is not as serious as it may at first appear is that
the majority of letters (as opposed to ligatures, and symbols)
that occur in LY1 occur in the same place in T1.

The only letters that might possibly appear in a hyphenation
table that are in different positions in T1 and LY1 are:

\oe  (low position OT1 high new)
\ss  (low position OT1 high new)
\v{s}
\v{z}
\l
\i   OT1  (although *composites* such as \'\i are in T1 position
           so this will only affect languages (Turkish?) that use
           an unaccented \i)
\"{y}


It should be noted that for those symbols that occur twice in
LY1, the `high' copy is used if it coincides with the position
used in T1 (as in the case of \ae, \o) otherwise the `low'
copy will be used which will coincide with the OT1 position
(\oe, \ss).  (Unless the setup for ansinew is enabled in which
case the high position is always used.)

Fortunately most hyphenation files for Western European
languages (I checked French, German and Danish) duplicate all
the hyphenation patterns using these letters so that the
tables work with both T1 and OT1 (and hence LY1) encoded
fonts.  However if you are using a language that makes use of
say, \ss, but the hyphenation patterns just refer to \ss as
^^ff then you will need to copy the hyphenation file and edit
all occurrences of ^^ff to refer to the new position; either
^^19 (for texnansi) or ^^df (for ansinew).

The remaining letters that are in different positions, such as
s caron, may be dealt with similarly, although they are mainly
used in Eastern European languages.  The LY1 encoding does not
have as many glyphs for Eastern European languages as T1, so
for those languages most likely this encoding is not suitable.
(Of course TeX can produce all the accented letters required,
but the hyphenation algorithm can not work with such
constructed composites it can only work with composite letters
that actually occur in the font.)

It would be a good thing if hyphenation tables did not refer
to any explicit character positions using the ^^ab notation,
but rather always accessed characters by control sequences
such as \ss.  This would allow the remapping to be done via
inputting a file such as ly1enc.def rather than by editing the
hyphenation file.  However currently most of the publicly
available hyphenation tables unfortunately do `hard wire' the
T1 character codes in this way.


Copyright 1997 David Carlisle
(Updated Feb. 2001 Walter Schmidt)
(Updated Jun. 2010 Karl Berry)
(Updated Oct. 2010 Karl Berry -- Times small caps faked as intended.)
(Updated Jan. 2011 Karl Berry
 -- missing map entries for ptmrr8ye and ptmr8yn.
 -- irrelevant {phvl*,psyr,pzdr}.tfm removed.
 -- relevant ptm{b,r}c8y.vf included, and corresponding ptm{b,r}c8y.tfm.
 Thanks to Bruno Voisin for much research and debugging.
)


All the files in this directory may be redistributed and/or modified
under the terms of the LaTeX Project Public License 
http://www.latex-project.org/lppl/
either version 1 of the License, or (at your option) any later version.


==> ly1/doc/fonts/ly1/README <==
LaTeX support for `texnansi' encoding (LY1)
===========================================

Installing
==========

Ordinarily, you don't have to do anything, since this package is likely
already present in your TeX distribution (TeX Live, MiKTeX).

But if you're on your own, then just recursively copy the directories
here to your texmf-local (or some) tree, preserving structure.  Then add
the map files *8y.map to your dvips setup and/or update the
configuration of other DVI drivers correspondingly.  You will have to
adjust URW vs. Adobe names as needed.  (In TeX Live, this is already
done in dvips35.map, etc., in conjunction with updmap, and the *8y.map
files here are not used.)

Usage
=====

The font encoding `LY1' corresponds to the `texnansi' encoding as used
by default in the Y&Y TeX system (http://tug.org/yandy).  There is also
an option to support the `ansinew' encoding that is the default encoding
in Microsoft Windows.

The main file is ly1enc.def. This contains the declaration of
the encoding. To use `texnansi' encoded fonts within LaTeX, 
typically you just need to add the line

	\usepackage[LY1]{fontenc}

to your document preamble.

An alternative to the above line is to use the `texnansi' package

	\usepackage{texnansi}

This will call the fontenc package, as above, to set up the LY1
encoding but then make further changes to the uppercase and
lowercase tables.  Note that LaTeX does not need these changes to
correctly uppercase text as its \MakeUppercase and \MakeLowercase
commands only require the uppercase and lower case codes of the
letters a-z.

So for most purposes it is better to use the call to fontenc
rather than use the `texnansi' package.  Then, if you pass the
file to a site using T1 (Cork) encoded fonts the line can more
easily be changed to

	\usepackage[T1]{fontenc}

The texnansi package has a package option `ansinew' which
modifies the LY1 encoding to refer to that MS Windows
encoding.  However you should only do this if your TeX system
can not reencode fonts to support T1 or LY1.  The `ansinew'
treatment of the left quote ` as a grave accent makes it
rather unsuitable for TeX use.  It also lacks several useful
glyphs.  However if you need to, you can do:

	\usepackage[ansinew]{texnansi}

The other possible reason for using the `texnansi' package
relates to the use of the lowercase table in the hyphenation
algorithm.  This is described below, but it is unfortunately
of necessity rather technical, and you may want to stop
reading at that point.

LY1 matches OT1 well enough that you can usually use it in that role
also.  You can \input texnansi if you want this to work exactly even in
plain TeX.

Having declared the LY1 encoding to LaTeX, LaTeX will need to
know the fonts that are available in this encoding.  This
distribution includes TeX metrics, font definition files and
map files for the common `Standard PostScript' fonts.

For each encoding LaTeX needs to know an `error font' which is
its fall back in the case that the font substitution system
can find nothing better to do.  ly1enc.def specifies that the
Error Font for LY1 is Adobe Times-Roman.  Any PostScript
interpreter must be able to provide Times-Roman, so it seems a
good choice as the error font.  Yet you may wish to change
this for any reason; just edit the lines

\DeclareErrorFont{LY1}{ptm}{m}{n}{10}
\DeclareFontSubstitution{LY1}{ptm}{m}{n}

at the top of ly1enc.def to refer to some other font set.  For example
if you have Y&Y TeX's `Lucida Bright' distribution you could change the
two occurrences of {ptm} to {hlh} to make LaTeX fall back on Lucida
Bright if all else fails.  Please follow the LPPL and do not
capriciously alter ly1enc.def in other ways.

For more information on LY1 encoding and see Y&Y's WWW page:

        <http://www.tug.org/yandy/usely1.htm>
        

A Note on Lowercase Codes and Hyphenation Tables
================================================

The lowercase table is used by TeX's hyphenation algorithm, so
in principle one would need to change the lowercase table to
match the encoding used.  However, it should not be changed
mid paragraph as all words, whatever font encoding they are
set in, are lowercased using the table current at the *end* of
the paragraph before being checked for hyphenation.  Because
of these limitations in TeX's hyphenation algorithm, LaTeX
does not support changing the lowercase table mid document, so
if the `texnansi' package is used then the `texnansi'
lowercase table will be used for all fonts (whether or not LY1
encoded) and conversely if it is not used, the T1 table will
be used, even for LY1 encoded fonts.  The reason why this
problem is not as serious as it may at first appear is that
the majority of letters (as opposed to ligatures, and symbols)
that occur in LY1 occur in the same place in T1.

The only letters that might possibly appear in a hyphenation
table that are in different positions in T1 and LY1 are:

\oe  (low position OT1 high new)
\ss  (low position OT1 high new)
\v{s}
\v{z}
\l
\i   OT1  (although *composites* such as \'\i are in T1 position
           so this will only affect languages (Turkish?) that use
           an unaccented \i)
\"{y}


It should be noted that for those symbols that occur twice in
LY1, the `high' copy is used if it coincides with the position
used in T1 (as in the case of \ae, \o) otherwise the `low'
copy will be used which will coincide with the OT1 position
(\oe, \ss).  (Unless the setup for ansinew is enabled in which
case the high position is always used.)

Fortunately most hyphenation files for Western European
languages (I checked French, German and Danish) duplicate all
the hyphenation patterns using these letters so that the
tables work with both T1 and OT1 (and hence LY1) encoded
fonts.  However if you are using a language that makes use of
say, \ss, but the hyphenation patterns just refer to \ss as
^^ff then you will need to copy the hyphenation file and edit
all occurrences of ^^ff to refer to the new position; either
^^19 (for texnansi) or ^^df (for ansinew).

The remaining letters that are in different positions, such as
s caron, may be dealt with similarly, although they are mainly
used in Eastern European languages.  The LY1 encoding does not
have as many glyphs for Eastern European languages as T1, so
for those languages most likely this encoding is not suitable.
(Of course TeX can produce all the accented letters required,
but the hyphenation algorithm can not work with such
constructed composites it can only work with composite letters
that actually occur in the font.)

It would be a good thing if hyphenation tables did not refer
to any explicit character positions using the ^^ab notation,
but rather always accessed characters by control sequences
such as \ss.  This would allow the remapping to be done via
inputting a file such as ly1enc.def rather than by editing the
hyphenation file.  However currently most of the publicly
available hyphenation tables unfortunately do `hard wire' the
T1 character codes in this way.


Copyright 1997 David Carlisle
(Updated Feb. 2001 Walter Schmidt)
(Updated Jun. 2010 Karl Berry)
(Updated Oct. 2010 Karl Berry -- Times small caps faked as intended.)
(Updated Jan. 2011 Karl Berry
 -- missing map entries for ptmrr8ye and ptmr8yn.
 -- irrelevant {phvl*,psyr,pzdr}.tfm removed.
 -- relevant ptm{b,r}c8y.vf included, and corresponding ptm{b,r}c8y.tfm.
 Thanks to Bruno Voisin for much research and debugging.
)


All the files in this directory may be redistributed and/or modified
under the terms of the LaTeX Project Public License 
http://www.latex-project.org/lppl/
either version 1 of the License, or (at your option) any later version.


==> ly1/tex/plain/ly1/texnansi.tex <==
% Copyright 2010--2018 TeX Users Group.
% Copyright 1994--1997 Y&Y, Inc.

% Released under the LaTeX Project Public License, any version.

% ============================================================================
% Code to allow plain TeX and LaTeX to fully exploit `texnansi.vec' encoding
%		(TeX 'n ANSI)	VERSION 2.8 (2018 May 25)
% ============================================================================

% \input texnansi in TeX source when using fonts with `TeX n ANSI' encoding.

% Note that a lot of code that already exists in plain.tex is commented out
% --- it is included here merely for reference.

% `plain' TeX - and `lplain' TeX - have accents hard-wired to certain codes.
% When a font is encoded differently, compound characters and accents move.
% This file deals with this for TeX 'n ANSI encoding.

% NOTE:  Default is to use the 58 ready-made accented/composite characters
% that occur in text fonts directly, using the macros defined below.
% To instead build them by overprinting, use \buildcomposites.
% To instead link to them via pseudo ligatures, use \usecomposites.

% NOTE: texnansi.vec is designed to avoid char codes 0, 9, 10, 13, 32, 127
% since some brain-dead software has trouble with some of these...

% NOTE: definitions have embedded numbers that depend on the chosen encoding
% These will need to be changed if you use an encoding other than `TEXNANSI'

% --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- ---
% First, protect against style files that make quotedbl `active'

\chardef\dblcode=\catcode`\"	% save catcode of quotedbl
\catcode`\"=12			% make quotedbl `other'

\chardef\atcode=\catcode`\@	% save catcode of atsign
\catcode`\@=11			% make atsign `letter'
% --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- ---

% NOTE: plain TeX (and LaTeX) has the accent character positions hardwired to:

% 16 for `dotlessi',	   17 for `dotlessj',	18 for `grave',	
% 19 for `acute',	   20 for `caron',	21 for `breve',	
% 22 for `macron',	   23 for `ring',	24 for `cedilla',
% 25 for `germandbls',	   26 for `ae',		27 for `oe',
% 28 for `oslash',	   29 for `AE',		30 for 'OE',	
% 31 for `Oslash',	   94 for `circumflex',	95 for `dotaccent',
% 125 for `hungarumlaut',  126 for `tilde',	127 for `dieresis',
% The *real* troublesome ones are `dotaccent' and `hungarumlaut'
% --- and CM fonts do not have `ogonek' --- which we add here.
% (see page 356 of the TeX book for additional information)

% --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- ---

% \ae, \oe, \o, \AE, \OE, \O, \ss are in same place as in TeX text

% Following constructed from pieces in CM, but exist in Type 1 text fonts

\def\aa{^^e5} \def\AA{^^c5}		% aring (229), Aring (197)
% \def\cc{^^e7} \def\CC{^^c7}		% ccedilla (231), Ccedilla (199)

% NOTE: \cc may conflict with `carbon copy' in letter.sty ...

\def\l{^^90} \def\L{^^80}		% lslash (144), Lslash (128)

% TEXNANSI also has the Icelandic characters:

\def\th{^^fe} \def\TH{^^de}		% thorn (254), Thorn (222)
\def\dh{^^f0} \def\DH{^^d0}		% eth (240), Eth (208)

\def\pounds{^^a3}	\def\copyright{^^a9}	% 163 and 169
\def\registered{^^ae}	\def\trademark{^^99}	% 174 and 153
% \def\dag{^^86}	\def\ddag{^^87}	% dagger (134), daggerdbl (135)
\def\S{^^a7}		\def\P{^^b6}	% section (167), paragraph (182)

% Make it more convenient to use { } _ | \ glyphs direct from text font ?

% \chardef\{=`\{ \chardef\}=`\} \chardef\_=`\_
% \chardef\|=`\| \chardef\backslash=`\\

% --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- ---

% Following set up for the 58 accented characters/composites in text fonts:

% aacute, acircumflex, adieresis, agrave, aring, atilde, ccedilla,
% eacute, ecircumflex, edieresis, egrave, iacute, icircumflex,
% idieresis, igrave, ntilde, oacute, ocircumflex, odieresis, ograve, otilde,
% scaron, uacute, ucircumflex, udieresis, ugrave, yacute, ydieresis, zcaron,
% Aacute, Acircumflex, Adieresis, Agrave, Aring, Atilde, Ccedilla,
% Eacute, Ecircumflex, Edieresis, Egrave, Iacute, Icircumflex,
% Idieresis, Igrave, Ntilde, Oacute, Ocircumflex, Odieresis, Ograve, Otilde,
% Scaron, Uacute, Ucircumflex, Udieresis, Ugrave, Yacute, Ydieresis, Zcaron,

\def\`#1{% grave
\if#1a^^e0\else%	\char224 
\if#1e^^e8\else%	\char232 
\if#1i^^ec\else%	\char236 
\if#1o^^f2\else%	\char242 
\if#1u^^f9\else%	\char249 
\if#1A^^c0\else%	\char192 
\if#1E^^c8\else%	\char200 
\if#1I^^cc\else%	\char204 
\if#1O^^d2\else%	\char210 
\if#1U^^d9\else%	\char217 
% \if#1{\i}^^ec\else%	\char236 
\if#1\i^^ec\else%	\char236 
{\accent18 #1}%
\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi}

\def\'#1{% acute
\if#1a^^e1\else%	\char225 
\if#1e^^e9\else%	\char233
\if#1i^^ed\else%	\char237
\if#1o^^f3\else%	\char243 
\if#1u^^fa\else%	\char250 
\if#1y^^fd\else%	\char253 
\if#1A^^c1\else%	\char193 
\if#1E^^c9\else%	\char201 
\if#1I^^cd\else%	\char205 
\if#1O^^d3\else%	\char211 
\if#1U^^da\else%	\char218 
\if#1Y^^dd\else%	\char221 
% \if#1{\i}^^ed\else%	\char237 
\if#1\i^^ed\else%	\char237 
{\accent19 #1}%
\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi}

\def\^#1{% circumflex
\if#1a^^e2\else%	\char226 
\if#1e^^ea\else%	\char234 
\if#1i^^ee\else%	\char238 
\if#1o^^f4\else%	\char244 
\if#1u^^fb\else%	\char251 
\if#1A^^c2\else%	\char194 
\if#1E^^ca\else%	\char202 
\if#1I^^ce\else%	\char206 
\if#1O^^d4\else%	\char212 
\if#1U^^db\else%	\char219 
% \if#1{\i}^^ee\else%	\char238 
\if#1\i^^ee\else%	\char238 
{\accent94 #1}%
\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi}

\def\~#1{% tilde
\if#1a^^e3\else%	\char227 
\if#1n^^f1\else%	\char241 
\if#1o^^f5\else%	\char245 
\if#1A^^c3\else%	\char195 
\if#1N^^d1\else%	\char209 
\if#1O^^d5\else%	\char213 
{\accent126 #1}%
\fi\fi\fi\fi\fi\fi}

\def\"#1{% dieresis
\if#1a^^e4\else%	\char228 
\if#1e^^eb\else%	\char235 
\if#1i^^ef\else%	\char239 
\if#1o^^f6\else%	\char246 
\if#1u^^fc\else%	\char252 
\if#1y^^ff\else%	\char255 
\if#1A^^c4\else%	\char196 
\if#1E^^cb\else%	\char203 
\if#1I^^cf\else%	\char207 
\if#1O^^d6\else%	\char214 
\if#1U^^dc\else%	\char220 
\if#1Y^^9f\else%	\char159 
% \if#1{\i}^^ef\else%	\char239 
\if#1\i^^ef\else%	\char239 
% {\accent127 #1}%
{\accent168 #1}%
\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi}

\def\v #1{% caron
\if#1s^^9a\else%	\char154 
\if#1z^^9d\else%	\char157 
\if#1S^^8a\else%	\char138 
\if#1Z^^8d\else%	\char141 
{\accent20 #1}%
\fi\fi\fi\fi}

\def\r #1{% ring
\if#1a^^e5\else%	\char229 
\if#1A^^c5\else%	\char197 
{\accent23 #1}%
\fi\fi}

\def\c #1{% cedilla
\if#1c^^e7\else%	\char231 
\if#1C^^c7\else%	\char199 
{\setbox0\hbox{#1}\ifdim\ht0=1ex\accent24 #1%
  \else{\ooalign{\hidewidth\char24\hidewidth\crcr\unhbox0}}\fi}%
\fi\fi}

\def\H#1{{\accent6 #1}}%	 hungarumlaut	% not in 125
\def\u#1{{\accent21 #1}}%	 breve

% dotaccent and macron have to be treated differently in AMS TeX

\ifx\amstexloaded@\relax%
\def\D#1{{\accent5 #1}}		% dotaccent	% not in 95
\def\B#1{{\accent22 #1}}	% macron
\let\graveaccent\`
\let\acuteaccent\'
\let\tildeaccent\~
\let\hataccent\^
\let\underscore\_
\else
\def\.#1{{\accent5 #1}}		% dotaccent	% not in 95
\def\=#1{{\accent22 #1}}\fi	% macron

% underline (using macron at 22)
\def\b#1{\oalign{#1\crcr\hidewidth
    \vbox to.2ex{\hbox{\char22}\vss}\hidewidth}}%

% ogonek (using ogonek at 7)
\def\k#1{\setbox0\hbox{#1}\ifdim\ht0=1ex\accent7 #1%
  \else{\ooalign{\hidewidth\char7\hidewidth\crcr\unhbox0}}\fi}%

% --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- ---

% For backward compatability, provide for use of font with TeX's \accent:
% (It is however generally better to use ready-made accented characters, since
% \accent creates explicit kerning, which breaks the hyphenation machinery)
% NOTE: Use \buildcomposites only if you want to force accented/composite
% characters to be constructed by `overprinting' base and accent.

\def\buildcomposites{%
% following four lines are for TeX n ANSI encoding only
\def\.##1{{\accent5 ##1}}%	 dotaccent	% not in 95
\def\H##1{{\accent6 ##1}}%	 hungarumlaut	% not in 125
\def\k##1{{\accent7 ##1}}%	 ogonek		% not in CM fonts
\def\"##1{{\accent168 ##1}}%	 dieresis	% alternate to 127
% following are plain TeX defaults (needed only to undo \usecomposites)
\def\`##1{{\accent18 ##1}}%	 grave
\def\'##1{{\accent19 ##1}}%	 acute
\def\^##1{{\accent94 ##1}}%	 circumflex
\def\~##1{{\accent126 ##1}}%	 tilde
\def\=##1{{\accent22 ##1}}%	 macron
\def\v##1{{\accent20 ##1}}%	 caron
\def\u##1{{\accent21 ##1}}%	 breve
% \def\"##1{{\accent127 ##1}}%	 dieresis	% use 168 instead
% underline and cedilla accents (macron at 22, cedilla at 24)
\def\b##1{\oalign{##1\crcr\hidewidth
    \vbox to.2ex{\hbox{\char22}\vss}\hidewidth}}%
\def\c##1{\setbox0\hbox{##1}\ifdim\ht0=1ex\accent24 ##1%
  \else{\ooalign{\hidewidth\char24\hidewidth\crcr\unhbox0}}\fi}%
}

% --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- ---

% USING READY-MADE ACCENTED CHARACTERS:
% We can also use pre-built accented character using pseudo ligatures ---
% provided the TFM files for the text fonts have them wired in.
% The following assumes that the TFM files have the required pseudo-ligatures.
% Use -vadj on the command line with AFMtoTFM to set up these pseudo-ligatures.
% This only works for the 58 ready-made accented/composite characters.

\def\usecomposites{%
\chardef\`=18	% grave
\chardef\'=19	% acute
\chardef\^=94	% circumflex
\chardef\~=126	% tilde
\chardef\"=127	% dieresis	% must match TFM, hence do *not* use 168 here
\chardef\c=24	% cedilla	% only for ccedilla, Ccedilla
\chardef\v=20	% caron		% only for scaron, zcaron, Scaron, Zcaron
\chardef\r=23	% ring		% non-standard, for Aring and aring
% and some extra goodies
\chardef\.=5	% dotaccent	% no standard accented chars use this
\chardef\H=6	% hungarumlaut	% no standard accented chars use this
\chardef\k=7	% ogonek	% no standard accented chars use this
\chardef\u=21	% breve		% no standard accented chars use this
\chardef\==22	% macron	% no standard accented chars use this
% \chardef\i=16	% dotlessi
}

% NOTE: To use the above scheme, use \'a, NOT \'{a}, and \c c, NOT \c{c}.

% --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- ---

% \buildcomposites	% build composites by overprinting base and accent
% \usecomposites	% use 58 ready-made composites via pseudo ligatures

% Default is to use 58 ready-made composites, and build others by overprinting.

% --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- --- ---

% Changes required in math macros when roman font is reencoded to `texnansi'.
% (An alternative is to draw the accents from the math fonts)

% Most accents are in same place as in TeX text encoding (except dotaccent)

\def\usetextaccents{
% \def\grave{\mathaccent"7012 }	%  18 grave
% \def\acute{\mathaccent"7013 }	%  19 acute
% \def\hat{\mathaccent"705E }	%  94 circumflex
% \def\tilde{\mathaccent"707E }	% 126 tilde
% \def\ddot{\mathaccent"707F }	% 127 dieresis
\def\ddot{\mathaccent"70A8 }	% 168 dieresis
% \def\bar{\mathaccent"7016 }	%  22 macron
% \def\check{\mathaccent"7014 }	%  20 caron
% \def\breve{\mathaccent"7015 }	%  21 breve
\def\dot{\mathaccent"7005 }	%   5 dotaccent
}

% Do not redefine accents in math mode when using MathTime,
% since MathTime uses accents in the math fonts - not those in the text font

% In LaTeX 2e check whether mathtime package has been loaded,
% otherwise check whether \MTMI is defined

\ifx\@ifpackageloaded\undefined\ifx\MTMI\undefined\usetextaccents\fi
\else\@ifpackageloaded{mathtime}{}{\usetextaccents}\fi

% **************************************************************************

% If you want to use < for `guilsinglleft' and > for `guilsinglright'
% then uncomment the following lines:

% \catcode`\<=\active \chardef<=139
% \catcode`\>=\active \chardef>=155

% If you use < for `exclamdown', > for `questiondown', and | for `emdash'
% then uncomment the following lines:

% \catcode`\<=\active \chardef<=161
% \catcode`\>=\active \chardef>=191
% \catcode`\|=\active \chardef|=151

% \chardef\lq=96 \chardef\rq=39

% Note that \lq and \rq also provide access to ` and '

\catcode`\@=\atcode		% restore original catcode of atsign

\catcode`\"=\dblcode		% restore original catcode of quotedbl

% If you use " for quotedblright then uncomment the following:

% \catcode`\"=\active \chardef"=148

% For proper hyphenation of words with accented characters we need to let
% TeX know how to translate words with accented characters to lower case.
% Hence define \lccode so that one can use them in \hyphenation{...}
% Just for fun, we also define \uccode, and set the \catcode to letter...

% Mostly in ISO Latin 1, accented characters (and a few special characters)
% occur in upper case form in the range 192 - 222, which is offset
% by 32 from the corresponding lower case forms in the range 224 - 254.

\bgroup
\newcount\n\newcount\m\n=224\m=192
\loop\ifnum\n<255
\global\catcode\n=11\global\catcode\m=11
\global\lccode\n=\n\global\lccode\m=\n
\global\uccode\m=\m\global\uccode\n=\m
\advance\n by1\advance\m by1\repeat
\egroup

% Then there are just a few odd ones in TEXNANSI that don't fit this pattern

\catcode140=11\catcode156=11	% OE, oe
\lccode140=156\lccode156=156
\uccode140=140\uccode156=140
\catcode159=11\catcode255=11	% Ydieresis, ydieresis
\lccode159=255\lccode255=255
\uccode159=159\uccode255=159
\catcode138=11\catcode154=11	% Scaron, scaron
\lccode138=154\lccode154=154
\uccode138=138\uccode154=138
\catcode141=11\catcode157=11	% Zcaron, zcaron
\lccode141=157\lccode157=157
\uccode157=141\uccode141=141
\catcode128=11\catcode144=11	% Lslash, lslash
\lccode128=144\lccode144=144
\uccode144=128\uccode128=128

\endinput

